Regular Variation in Hilbert Spaces and Principal Component Analysis for Functional Extremes

Motivated by the increasing availability of data of functional nature, we develop a general probabilistic and statistical framework for extremes of regularly varying random elements $X$ in $L^2[0,1]$. We place ourselves in a Peaks-Over-Threshold framework where a functional extreme is defined as an observation $X$ whose $L^2$-norm $\|X\|$ is comparatively large. Our goal is to propose a dimension reduction framework resulting into finite dimensional projections for such extreme observations. Our contribution is double. First, we investigate the notion of Regular Variation for random quantities valued in a general separable Hilbert space, for which we propose a novel concrete characterization involving solely stochastic convergence of real-valued random variables. Second, we propose a notion of functional Principal Component Analysis (PCA) accounting for the principal `directions' of functional extremes. We investigate the statistical properties of the empirical covariance operator of the angular component of extreme functions, by upper-bounding the Hilbert-Schmidt norm of the estimation error for finite sample sizes. Numerical experiments with simulated and real data illustrate this work.

==> Applications.tex <==
\subsection{Extreme Functional Linear Regression}
\textcolor{red}{il faut plus de motivations au problème comme dans article icml - attention résultats très (trop?) similaires à Section 5 de \cite{Xiong3}, à étudier plus en détails} Great review on Functional Regression (Linear :Scalar-on-Function, Function-on-Scalar, Function-on-Function; Non-Linear) :\cite{morris2015functional}, \cite{horvath2012inference}. 
Here, we are interested in the Functional Linear Model (FLM) with scalar responses (even if we can adapt our work to functional responses). Our inference method is based on technics used in \cite{imaizumi2018pca}. We consider the following model (FLM):
\begin{equation*}
Y = B_0 + \int_0^1 X(s) B(s) ds + \varepsilon,
\end{equation*}
where $Y$ is the scalar output, $B_0 = \bb{E}[Y]$ the intercept, $X$ the centered functional input, and $\varepsilon$ a zero-mean Gaussian noise independent from $X$. The goal is to estimate $B$. Here, we want to perform the regression in extreme regions, \ie in regions far from the origin here $\|X\|$ is 'large', then we assume that $X$ is regularly varying with index $-\alpha$ in $L^2([0,1])$ such that
\begin{equation*}
\mathcal{L}(\Theta_t):=\mathcal{L}\Big(\frac{X}{\|X\|} \mid \|X\| \s t\Big) \rightarrow \mathcal{L}(\Theta_\infty),
\end{equation*}
as $t \rightarrow +\infty$.
Then, the Extreme FLM problem turns out to be the following one
\begin{equation}\label{eq:ext_mod}
Y_\infty = B_{\infty,0} + \int_0^1 X_\infty(s) B_\infty(s)ds +\varepsilon.
\end{equation}
Since $\|X_\infty\|$ is $\alpha$-Pareto distributed and independent from $\Theta_\infty$, we can approach this model by the following one
\begin{equation}\label{eq:approx_ext_mod}
Y_t = B_{t,0} + P \int_0^1 \Theta_t(s) B_t(s) ds + \varepsilon,
\end{equation}
for $t$ large enough, $P$ $\alpha$-Pareto distributed independent from $X$, and with $\mathcal{L}(Y_t) = \mathcal{L}(Y \mid \|X\| \s t)$. However, $P$ is of no interest in this model, and thus the final model considered is the following
\begin{equation}\label{eq:approx_mod}
Y_t = B_{t,0} +  \int_0^1 \Theta_t(s) B_t(s) ds + \varepsilon.
\end{equation}

A classical way to estimate the linear regression function $B$ is first to approximate it by considering the truncation of its development according to an appropriate basis and then to estimate its coordinate coefficients in this basis. Unsurprisingly, the considered basis will be the basis generated by performing PCA on $\Theta_t$ for given $t$. We suppose that $\Theta_t$ is zero mean for all $t>0$. For a given $t$, we consider the Karhunen-Loève expansion of $\Theta_t$:
\begin{equation*}
\Theta_t = \sum_{i=1}^\infty Z_i^t \varphi_i^t,
\end{equation*}
with $Z_i^t = \langle \Theta_t,\varphi_i^t \rangle$ and $(\varphi_i^t)_{i \s 1}$ the principal components of $\Theta_t$. Since $(\varphi_i^t)_{i \s 1}$ forms an orthonormal basis of $L^2([0,1])$, we can expand $B_t$ according to this basis:
\begin{equation*}\label{eq:B_expansion}
B_t(s) = \sum_{i=1}^{+\infty} b_i^t \varphi_i^t(s),
\end{equation*}
for $t \in [0,1]$. Hence, equation (\ref{eq:approx_mod}) becomes
\begin{equation*}
Y_t = B_{t,0} + \sum_{i=1}^{+\infty} Z_i^t b_i^t +\varepsilon.
\end{equation*}
Following technics in \cite{imaizumi2018pca}, since for every $j\s 1$, $\bb{E}[Z_j^t] = 0$, we have:
\begin{equation}
\bb{E}[Z_j^t Y_t] = \E[(Z_j^t)^2]b_j^t \Leftrightarrow \ b_j^t = \frac{\bb{E}[Z_j^t Y_t]}{\E[(Z_j^t)^2]}. \label{eq:bt}
\end{equation}

%Consider a sample of inputs $(X_1,...,X_n)$ distributed as $X$ associated with a sample of output $(Y_1,...,Y_n)$. A natural estimate of $\varphi_j^{t_{n,k}}$ is given by $\hat{\varphi}_j^{\hat{t}_{n,k}}$ by performing PCA on the empirical thresholded covariance kernel function $\hat{C}_{\hat{t}_{n,k}}$ as in Section \ref{sec:stats}. Finally, a natural estimate of $b_i^{t_{n,k}}$ is given by
%\begin{align*}
%\hat{b}_j^{\hat{t}_{n,k}}&= \frac{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}}Y_i}{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle^2\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}}} \\
%&= \frac{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle\1\{\|X_i\|\s \hat{t}_{n,k}\}Y_i}{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle^2\1\{\|X_i\|\s \hat{t}_{n,k}\}}.
%\end{align*}

%Finally, an estimation/approximation of $B_{t_{n,k}}$ would be given by
%\begin{equation}
%\hat{B}^{m_{n,k}}_{\hat{t}_{n,k}}(s) = \sum_{i=1}^{m_{n,k}} \hat{b}_i^{\hat{t}_{n,k}} \hat{\varphi}_i^{\hat{t}_{n,k}}(s),
%\end{equation}
%with $m_{n,k}$ the number of basis functions used to approximate $B_{t_{n,k}}$ depending on the sample size $n$ and the number of extreme observations $k$ and such that $m_{n,k} \underset{k \rightarrow +\infty}{\longrightarrow} +\infty$.

\begin{remark} This framework can be adapted to function responses, in the same way as \cite{imaizumi2018pca}.
\end{remark}

\begin{remark}In our settings, we assume that the noise $\varepsilon$ is independent from $X$ but only $\E[X \varepsilon ] =0$ is mandatory to achieve our concluding results.
\end{remark}
It remains to prove how this estimated approximation is close to the $B$ involved in Equation (\ref{eq:ext_mod}). Article PCA-bsed estimation for scalar reponses \cite{hall2007methodology}.

\subsubsection{Deterministic convergence}
We can consider the Karhunen-Loève expansion of $\Theta_\infty$ (also zero mean since $\Theta_t$ is zero mean for all $t>0$)
\begin{equation}
\Theta_\infty(s) = \sum_{i=1}^{+\infty} Z_i^\infty \varphi_i^\infty(s),
\end{equation}
and in the same way than above, we can develop $B_\infty$ according to the KLE-basis of $\Theta_\infty$
\begin{equation}
B_\infty(s) = \sum_{i=1}^{+\infty} b_i^\infty \varphi_i^\infty(s),
\end{equation}
with $b_j^\infty = \bb{E}[Z_j^\infty Y_\infty]/\bb{E}[(Z_j^\infty)^2]$.
The main assumption during this study (recurrent hypothesis in articles of this kind) is the following one.

\textbf{\underline{Assumption (H.1)}}: the eigenvalues of the covariance of $\Theta_\infty$ are distinct
\begin{equation}
\lambda_\infty^1 > \lambda_\infty^2 >...>0. \tag{H.1}\label{hyp:H.1}
\end{equation}
To make this problem consistent, we have to suppose that the following distribution joint convergence holds.

\textbf{\underline{Assumption (H.2)}}: $|Y|$ is almost surely bounded by $M>0$ and there exists a real-valued bounded random variable $Y_\infty$ such that
\begin{equation}
\mathcal{L}(Y_t,\Theta_t) \tti \mathcal{L}(Y_\infty, \Theta_\infty). \tag{H.2} \label{hyp:H.2}
\end{equation}
\textbf{First question}: Can one have $m_{n,k}$ such that $B^{m_{n,k}}_{t_{n,k}} \overset{\|\cdot\|_2}{\longrightarrow} B_\infty$, as $k \rightarrow +\infty$?

The first step is to decompose the convergence and to consider the two intermediate quantities $B^m_\infty$ and $B_t$.
By definition, the two convergences hold true
\begin{equation}
B^m_t \underset{m \rightarrow +\infty}{\longrightarrow} B_t \text{ and } B_\infty^m\underset{m \rightarrow +\infty}{\longrightarrow} B_\infty,
\end{equation}
w.r.t. $\|\cdot\|_2$. With our assumptions, the following convergence also holds true.
\begin{proposition}\label{prop:5.1}For a fixed $m \in \bb{N}$,
\begin{equation*}
B_t^m \tti B_\infty^m,
\end{equation*}
w.r.t. $\|\cdot\|_2$.
\end{proposition}
Without any further assumption, it seems impossible to obtain a better result, \ie a "double-convergence" of $B^{m_{n,k}}_{t_{n,k}}$ toward $B_\infty$, since no convergence rates subsist for the extreme convergence of $B_{t_{n,k}}^m$ toward $B_\infty^m$ and approximation convergence of $B_t^{m_{n,k}}$ toward $B_t$ as $k \rightarrow +\infty$. 

%However, Assumption \ref{hyp:H.1.1} in the coming section offers
%\begin{proposition} There exists a sequence $(m_{n,k})$ such that
%\begin{equation}
%\|B_{t_{n,k}}^{m_{n,k}}-B_\infty\|_2 \rightarrow 0,
%\end{equation}
%as $k \rightarrow +\infty$.
%\end{proposition}
%\begin{proof}
%\textcolor{red}{todo, possible?}
%\end{proof}
\subsubsection{Probabilistic convergences}
In order to find an appropriate $m_{n,k}$, assumption (\ref{hyp:H.1}) is too vague, and an additional assumption is needed to precise how well-separated are the eigenvalues.

\textbf{\underline{Assumption (H.1.1)}}\label{hyp:H.1.1}: \textcolor{red}{peut-on affaiblir?} there exist two bounded sequences $(C_{1,k})$, $(C_{2,k})$ and two constants $\alpha, \beta > 1/2$ such that for all $k \s 1$ and $j \s 1$,
\begin{equation}
\lambda_j^{t_{n,k}}\m C_{1,k} j^{-\alpha}, \tag{H.1.1.a} \label{eq:H.1.1.a}
\end{equation}
\begin{equation}
\lambda_j^{t_{n,k}} - \lambda_{j+1}^{t_{n,k}}\s C_{1,k}^{-1} j^{-\alpha -1}, \tag{H.1.1.b}\label{eq:H.1.1.b}
\end{equation}
\begin{equation}
| b_j^{t_{n,k}}| \m C_{2,k} j^{-\beta}. \tag{H.1.1.c} \label{eq:H.1.1.c}
\end{equation}

\begin{remark}Assumptions (\ref{eq:H.1.1.a}) and (\ref{eq:H.1.1.b}) imply that $\lambda_j^{t_{n,k}}$ is exactly of order $j^{-\alpha}$ because 
\begin{equation}
\lambda_j^{t_{n,k}} = \sum_{i=j}^{+\infty}(\lambda_i^{t_{n,k}}-\lambda_{i+1}^{t_{n,k}})\s (C_{1,k}\alpha)^{-1} j^{-\alpha}.
\end{equation}
Notice that if $\alpha >1$ then $C_t$ is a trace-class operator for all $t >0$.
Since $(C_{1,k})$ and $(C_{2,k})$ are two bounded sequences, quantities related to the covariance operator $C_\infty$ also fulfill Assumption (\hyperref[hyp:H.1.1]{H.1.1}).
\end{remark}

\begin{remark} Assumption (\ref{eq:H.1.1.c}) entails that for all sequence $(u_k)$ such that $u_k \rightarrow +\infty$ as $k$ tends to infinity, we have
\begin{equation*}
\|B_{t_{n,k}}^{u_k} - B_{t_{n,k}}\|_2 \rightarrow 0,
\end{equation*}
as $k\rightarrow +\infty$.
\end{remark}
We denote by $\Delta_{n,k}:=\|C_{t_{n,k}}-\hat{C}_{\hat{t}_{n,k}}\|$ and introduce the event $\mathcal{E}(n,k):=\{\frac{1}{2}\lambda_{m_{n,k}}^{t_{n,k}} \s \Delta_{n,k} \}$. For some results, we have to work under the assumption that $\mathcal{E}(n,k)$ holds true to navigate from $\hat{\lambda}_{m_{n,k}}^{\hat{t}_{n,k}}$ to $\lambda_{m_{n,k}}^{t_{n,k}}$ and thus use freely hypothesis introduced above.

\begin{remark}\label{rem:5.4} We know by results from Section \ref{sec:KL} that $\Delta_{n,k} = O_\bb{P}(1/\sqrt{k})$. Hence, following hypothesis (\ref{eq:H.1.1.a}), if $\sqrt{k}m_{n,k}^{-\alpha} \rightarrow +\infty$, as $k \rightarrow +\infty$, it holds that $\bb{P}\{\mathcal{E}(n,k)\} \rightarrow 1$, as $k \rightarrow +\infty$. Observe that this hypothesis is useful to exploit the inequality $\hat{\lambda}_{m_{n,k}}^{\hat{t}_{n,k}} \s \frac{1}{2}\lambda_{m_{n,k}}^{t_{n,k}}$.
\end{remark}
The goal of this section is to find $m_{n,k}$ such that a computable estimator of $B_{t_{n,k}}^{m_{n,k}}$ fulfills $\| \hat{B} - B_{t_{n,k}}^{m_{n,k}}\|_2 \overset{\bb{P}}{\rightarrow} 0$. A natural approximating and estimating candidate for $\hat{B}$ is given by
\begin{equation}
\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}}:= \sum_{i=1}^{m_{n,k}} \hat{b}_i^{\hat{t}_{n,k}} \hat{\varphi}_i^{t_{n,k}},
\end{equation}
where $\hat{\varphi}_j^{t_{n,k}}$ is the $j$-th eigenfunction of the empirical thresholded covariance operator (as in Section \ref{sec:stats}) and, following Equation (\ref{eq:bt}),
\begin{align}
\hat{b}_j^{\hat{t}_{n,k}}&= \frac{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}}Y_i}{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle^2\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}}} \\
&= \frac{\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle\1\{\|X_i\|\s \hat{t}_{n,k}\}Y_i}{\sum_{l=1}^n \langle \Theta_l,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle^2\1\{\|X_l\|\s \hat{t}_{n,k}\}}.
\end{align}
\begin{remark} We assume that $\langle \hat{\varphi}_{j}^{\hat{t}_{n,k}}, \varphi_j^{t_{n,k}} \rangle \s 0$ in order to ensure that $\hat{\varphi}_{j}^{\hat{t}_{n,k}}$ is an estimator of $\varphi_j^{t_{n,k}}$.
\end{remark}
As in Section \ref{sec:KL}, probabilistic convergences is divided in two parts since
\begin{align}
\|\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}} - B_{t_{n,k}}^{m_{n,k}}\|_2^2 &= \| \sum_{i=1}^{m_{n,k}} \hat{b}_i^{\hat{t}_{n,k}} \hat{\varphi}_i^{\hat{t}_{n,k}}- \sum_{i=1}^{m_{n,k}} b_i^{t_{n,k}} \varphi_i^{t_{n,k}} \|_2^2 \nonumber \\
&= \| \sum_{i=1}^{m_{n,k}} (\hat{b}_i^{\hat{t}_{n,k}} - b_i^{t_{n,k}})\hat{\varphi}_i^{\hat{t}_{n,k}} + \sum_{i=1}^{m_{n,k}} b_i^{t_{n,k}}(\hat{\varphi}_i^{\hat{t}_{n,k}} - \varphi_i^{t_{n,k}}) \|_2^2 \nonumber \\
&\m 2\sum_{i=1}^{m_{n,k}} (\hat{b}_i^{\hat{t}_{n,k}} - b_i^{t_{n,k}})^2 + 2\Big(\sum_{i=1}^{m_{n,k}} | b_i^{t_{n,k}}|\|\hat{\varphi}_i^{\hat{t}_{n,k}} - \varphi_i^{t_{n,k}}\|_2 \Big)^2. \label{eq:decomp}
\end{align}

The two following propositions handle those probabilistic convergences.
\begin{proposition}\label{prop:6.2}
We have with probability at least $1-\delta/2$
\begin{align}
\Big(\sum_{i=1}^{m_{n,k}} |b_i^{t_{n,k}}|\|\hat{\varphi}_i^{\hat{t}_{n,k}} - \varphi_i^{t_{n,k}}\|_2 \Big)^2 \m \Big( 2\sqrt{2} C_{1,k}C_{2,k} \sum_{i=1}^{m_{n,k}}i^{\alpha - \beta +1}\Big)^2 &\Bigg(\frac{1}{\sqrt{k}}+\frac{4}{3k}\log(4/\delta)+4\bigg(\bigg(\frac{\log(4/\delta)}{3k}\bigg)^2+\frac{\log(4/\delta)}{k} \bigg)^{1/2} \nonumber \\
&+ \frac{1}{3k}\log(8/ \delta ) + \bigg( \bigg( \frac{\log (8/\delta)}{3k} \bigg)^2 + \frac{2\log(8/ \delta)}{k} \bigg)^{1/2}\Bigg)^2.
\end{align}
\end{proposition}
In order to handle the first term of Equation (\ref{eq:decomp}), we have once again to partition the work
\begin{equation}\label{eq:36}
(\hat{b}_j^{\hat{t}_{n,k}} - b_j^{t_{n,k}})^2 \m 2\Big((\hat{b}_j^{\hat{t}_{n,k}} - \Tilde{b}_j^{\hat{t}_{n,k}})^2+(\Tilde{b}_j^{\hat{t}_{n,k}} - b_j^{t_{n,k}})^2\Big),
\end{equation}
with
\begin{equation}
\Tilde{b}_j^{\hat{t}_{n,k}}:=\frac{1}{\hat{\lambda}_j^{\hat{t}_{n,k}}}\E [Z_j^{t_{n,k}}Y_{t_{n,k}}]=\frac{\lambda_j^{t_{n,k}}}{\hat{\lambda}_j^{\hat{t}_{n,k}}}b_j^{t_{n,k}}.
\end{equation}


\begin{lemma}\label{lemma:6.2}
If $\mathcal{E}(n,k)$ holds true, we have with probability $1-\delta/4$
\begin{multline*}
(\Tilde{b}_j^{\hat{t}_{n,k}} - b_j^{t_{n,k}})^2 \m (\alpha C_{1,k}C_{2,k})^2 j^{2(\alpha - \beta)}\Bigg(\frac{1}{\sqrt{k}}+\frac{4}{3k}\log(8/\delta)+4\bigg(\bigg(\frac{\log(8/\delta)}{3k}\bigg)^2+\frac{\log(8/\delta)}{k} \bigg)^{1/2} \\
+ \frac{1}{3k}\log(16/ \delta ) + \bigg( \bigg( \frac{\log (16/\delta)}{3k} \bigg)^2 + \frac{2\log(16/ \delta)}{k} \bigg)^{1/2}\Bigg)^2.
\end{multline*}
%
\end{lemma}

\begin{lemma}\label{lemma:6.1}\textcolor{red}{vrai mais il  faut refaire preuve comme dans \cite{hall2007methodology} pour avoir convergence rate voulu}
Let $\delta \in (0,1)$. If $\mathcal{E}(n,k)$ holds, we have with probability at least $1-\delta/4$
\begin{align*}
(\hat{b}_j^{\hat{t}_{n,k}} - \Tilde{b}_j^{\hat{t}_{n,k}})^2 \m 12M^2(C_{1,k}\alpha)^2j^{2\alpha}\Bigg(&\Big(\frac{1}{\sqrt{k}}+\frac{4}{3k}\log(12/\delta)+4\bigg(\bigg(\frac{\log(12/\delta)}{3k}\bigg)^2+\frac{\log(12/\delta)}{k} \bigg)^{1/2}\Big)^2 \\
&+ \Big(\frac{2}{3k}\log(24/ \delta ) + 2\bigg( \bigg( \frac{\log (24/\delta)}{3k} \bigg)^2 + \frac{2\log(24/ \delta)}{k} \bigg)^{1/2}\Big)^2 \\
&+ 8C_{1,k}^2 j ^{2\alpha+2}\Big(\frac{1}{\sqrt{k}}+\frac{4}{3k}\log(12/\delta)+4\bigg(\bigg(\frac{\log(12/\delta)}{3k}\bigg)^2+\frac{\log(12/\delta)}{k} \bigg)^{1/2}\Big)^2\Bigg).
\end{align*}
\end{lemma}
%\begin{proof}
%First, notice that for all $j\s 1$
%\begin{equation}
%\frac{1}{n}\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle^2\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}} = \hat{\lambda}_j^{\hat{t}_{n,k}}.
%\end{equation}
%Hence,
%\begin{align*}
%(\hat{b}_j^{\hat{t}_{n,k}} - \Tilde{b}_j^{\hat{t}_{n,k}})^2 &= \Big(\frac{1}{n}\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}}Y_i\Big)^2\Big(\frac{1}{\lambda_j^{t_{n,k}}}-\frac{1}{\hat{\lambda}_j^{\hat{t}_{n,k}}}\Big)^2 \nonumber \\
%&\m M^2\frac{1}{n}\sum_{i=1}^n \langle \Theta_i,\hat{\varphi}_j^{\hat{t}_{n,k}} \rangle^2\frac{\1\{\|X_i\|\s \hat{t}_{n,k}\}}{\frac{1}{n}\sum_{l=1}^n\1\{\|X_l\|\s \hat{t}_{n,k}\}} \Big(\frac{1}{\lambda_j^{t_{n,k}}}-\frac{1}{\hat{\lambda}_j^{\hat{t}_{n,k}}}\Big)^2 \nonumber \\
%&= M^2 \hat{\lambda}_j^{\hat{t}_{n,k}}\Big(\frac{\hat{\lambda}_j^{\hat{t}_{n,k}} - \lambda_j^{t_{n,k}}}{\lambda_j^{t_{n,k}}}\Big)^2 \nonumber \\
%&\textcolor{red}{\m} M^2 \Big(\frac{\|\hat{C}_{\hat{t}_{n,k}}- C_{t_{n,k}}\|_{HS}}{\lambda_j^{t_{n,k}}}\Big)^2. \nonumber
%\end{align*}
%Then, the result follows from Theorem \ref{thm:stats} and Assumption (\ref{eq:H.1.1.a}).
%\end{proof}

\begin{theorem}\label{thm:thm5.1}\textcolor{red}{(sans borne de concentration, on peut obtenir un meilleur résultat en suivant preuvede hall et horowitz, mais il faut rajouter des hypothèses) }Let $\delta \in (0,1)$. If $\mathcal{E}(n,k)$ holds, we have with probability at least $1-\delta$
\begin{equation}
\|\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}} - B_{t_{n,k}}^{m_{n,k}}\|_2^2 = O\Big((C_{1,k}C_{2,k})^2m_{n,k}^{2(\alpha-\beta)+1} k^{-1}+C_{1,k}^4 m_{n,k}^{4\alpha+3}k^{-1}+\big(C_{1,k}C_{2,k} \sum_{i=1}^{m_{n,k}}i^{\alpha - \beta +1}\big)^2k^{-1}\Big),
\end{equation}
\ie
\begin{equation}
\|\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}} - B_{t_{n,k}}^{m_{n,k}}\|_2^2 = O_{\bb{P}}\Big((C_{1,k}C_{2,k})^2m_{n,k}^{2(\alpha-\beta)+1}k^{-1}+C_{1,k}^4 m_{n,k}^{4\alpha+3}k^{-1}+\big(C_{1,k}C_{2,k} \sum_{i=1}^{m_{n,k}}i^{\alpha - \beta +1}\big)^2k^{-1}\Big).
\end{equation}
\end{theorem}

\begin{corollary}Let $\delta \in (0,1)$. Suppose that $(C_{1,k})$ and $(C_{2,k})$ are two convergent sequences. Then, we have
\begin{equation*}
\|\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}} - B_{t_{n,k}}^{m_{n,k}}\|_2^2 = O_{\bb{P}}\big(m_{n,k}^{4\alpha+3}k^{-1}+m_{n,k}^{2\alpha-2\beta+3}k^{-1}\big).
\end{equation*}
In particular, if $m_{n,k} = o(\min(k^{\frac{1}{4\alpha+3}},k^{\frac{1}{2\alpha-2\beta+3}}))$, we
\begin{equation*}
\|\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}} - B_{t_{n,k}}^{m_{n,k}}\|_2 =O_{\bb{P}}(1),
\end{equation*}
as $k \rightarrow +\infty$.
\end{corollary}

\begin{remark} In order to have $\sqrt{k}m_{n,k}^{-\alpha} \rightarrow + \infty$ as mentioned in Remark \ref{rem:5.4}, we should consider $m_{n,k} = o(\min(k^{\frac{1}{2\alpha}},k^{\frac{1}{2\alpha-2\beta+3}}))$ leading to $m_{n,k} = o(\min(k^{\frac{1}{4\alpha+3}},k^{\frac{1}{2\alpha-2\beta+3}}))$ since $4\alpha +3 >2\alpha$.
\end{remark}

Finally, given a new observation $X_{n+1}$ and knowing that $\|X_{n+1}\|$ is large enough (\ie $\|X_{n+1}\| \s \|X_{(k)}\|$), we may be interested in predictive performances of our estimator (as in \cite{crambes2009smoothing} or \cite{crambes2013asymptotics} for instance). Our estimator immediately gives the following estimated prediction
\begin{equation*}
\hat{Y}_{n+1}= \hat{B}_{\hat{t}_{n,k},0}+\int_0^1 \Theta_{n+1}(s) \hat{B}_{\hat{t}_{n,k}}^{m_{n,k}}(s)ds,
\end{equation*}
with $\hat{B}_{\hat{t}_{n,k},0} = \frac{1}{k}\sum_{i=1}^n Y_i \1\{\|X_i\| \s \hat{t}_{n,k}\}$ the natural estimate of the mean of $Y$ given $\|X\|$ large. Prediction error would ensue from the Cauchy-Schwartz inequality
\begin{equation*}
| Y_{n+1}-\hat{Y}_{n+1}| \m |\hat{B}_{\hat{t}_{n,k},0} - B_{t_{n,k},0}| + \|\hat{B}_{\hat{t}_{n,k}}^{m_{n,k}} - B_{t_{n,k}}\|,
\end{equation*}
and is controlled in probability by above results since $|\hat{B}_{\hat{t}_{n,k},0} - B_{t_{n,k},0}| = O_{\bb{P}}(1/\sqrt{k})$ (easy-to-show with the same maths as proof of Lemma \ref{lemma:6.1}).\textcolor{red}{section 8.6: integrated $R^2$-coeff to evaluate goodness of fit}

\subsection{Second Application (Anomaly detection?)}

\textcolor{red}{procedure à la damex en prenant comme données les scores de chaque observations (coordonnées dans kl-base)- data depth pour determiner si une observation est anormale ou non à partir des scores? ou classification? voir\cite{shang2014survey}}
Our algorithm is meant to detect anomalies among extreme regions, the most likely areas to contain abnormal observations. However, for the sake of completeness and precision, another classical anomaly detection analysis has to be performed to handle non-extreme anomalies (see Remark \ref{rem:11}).
\textbf{Proposition d'algo non supervisé:}

\begin{algorithm}[h] \label{algo1}
   \caption{Functional anomaly detection algorithm}
\begin{algorithmic}
   \STATE {\bfseries Inputs:} Dataset $\mathcal{D}_n=(\Tilde{X}_1,...,\Tilde{X}_n) \in (\bb{R}^{N_1})^n$ with $\Tilde{X}_j$ a dense discrete observation of a functional data;  number $k\leq n$ of 'extreme' observations; number $m$ of principal components kept for the study; a well-suited Hilbert basis $(e_i)_{i\s 1}$; number $N_2$ of interpolating functions, a well-chosen scoring function $\psi$.
   	\STATE {\bfseries Interpolation/Smoothing:} Compute the function $X_j = \sum_{i=1}^{N_2} x_{ji}e_i \in L^2([0,1])$ resulting from an interpolation/smoothing of $\Tilde{X}_j$ with $N_2$ basis functions of $(e_i)_{i\s 1}$.
	\STATE {\bfseries Functional Coordinate Standardization:} Standardize the coordinate vectors by means of the transformation $\hat{V}_j= \sum_{i=1}^{N_2} \hat{T}(x_j)_i e_i$ for $j=1,...,n$ where $\hat{T}(x_j) = \Big( \frac{1}{1-\hat{F}_1(x_{j1})},...,\frac{1}{1-\hat{F}_{N_2}(x_{jN_2})}\Big)$ with $x_j = (x_{j1},...,x_{jN_2})$ and $\hat{F}_i(x) = \frac{1}{n+1}\sum_{j=1}^n \1\{x_{ji} \m x\}$ an empirical cdf of $x_{\cdot i}$.
	\STATE {\bfseries Truncation:} Sort the data by decreasing order of magnitude $\| \hat{V}_{(1)}\| \s ... \s \|\hat{V}_{(n)}\|$ and keep only the $k$ largest angles of these observations $\{\Theta_1,...,\Theta_k\}$ with $\Theta_j = \hat{V}_{(j)} / \|\hat{V}_{(j)}\|$.
	\STATE {\bfseries Karhunen-Loève expansion:} Compute the $m_{n,k}$ first Karhunen-Loève eigenfunctions $(\varphi_1,..., \varphi_{m})$ (w.r.t. the basis $(e_i)_{i \s 1}$) according to the remaining sample $\{\Theta_1,...,\Theta_k\}$ and store the scores $\alpha_j = (\langle \Theta_j,\varphi_1 \rangle ,...,\langle \Theta_j,\varphi_{m} \rangle)$ for $ j = 1,...,k$.
	\STATE  {\bfseries Normality score:} Compute normality scores associated to each score $\alpha$ according to the scoring function $\psi$.
\STATE {\bfseries Outputs:} Outliers among extreme observations.
\end{algorithmic}
\end{algorithm}
A particular care should be taken not to be confused by scores stemmed from the Karhunen-Loève procedure, \ie coordinates in the KL-basis, and normality scores representing degree of normality of an observation, \ie outputs of the scoring function. A few remarks are in order.
\begin{remark}{(\sc Functional Marginal Standardization)} The coordinate standardization used in the algorithm is only relevant because functions are dived into a finite dimensional space. Observe that an application without any adjustment of this transformation on truly infinite-dimensional functions is impossible: the resulting function would not even belong to $L^2([0,1])$. Define correctly a functional marginal transformation (even in the continuous path case) is much more difficult than in finite dimension because of the need of conservation of regularity conditions (integrability, continuity,...) and relative compactness/tightness conditions.
\end{remark}

\begin{remark}{(\sc What is the benefit of this procedure?)} A natural question to ask is "Why would one not work straightforwardly	with $(\Tilde{X}_1,...,\Tilde{X}_n)$?". This question can merely be restated in an unambiguous and enlightening manner "Why Functional Data Analysis?". Typical reasons for considering functional data is to exploit properties of a potential regular structure (continuity, derivability, integrability...) conducting to a more accurate study or simply to avoid high-dimensional issues when $N_1 \gg n$. The reader is invited to read first pages of \cite{FDA} (or any books about FDA) to have a more complete picture of underlying issues of FDA. Second, an other natural question arises "Why does one not compute normality scores w.r.t. coordinates in the $(e_i)_{i \s 1}$ basis?". Even with a careful choice of the basis $(e_i)_{i\s 1}$, the Karhunen-Loève basis remains the best linear approximation basis (see the very instructive Chapter 9 of \cite{mallat2000exploration}) and as a result, it allows to properly reduce the dimension of the data.
\end{remark}

\begin{remark}{ (\sc Choice of Normality function)} For the computation of final normality scores, two options are available. First, a functional data depth (or any application delivering a normality score from a functional data) could be used to compute the normality score using the Karhunen-Loève expansion of each observation. Authors in \cite{gijbels2017general} display an instructive and exhaustive comparison between functional data depths which may help the reader to select an appropriate depth for its concern. The second alternative is to consider only scores associated to each Karhunen-Loève expansion and then to employ a multivariate method to compute normality scores. Multivariate data depths could of course be used (see \textcolor{red}{review mv depth}) but the DAMEX algorithm (see \cite{DAMEX}) seems well suited to handle the problem. Regarding  The first option appears more natural to yield better result since more information is retained in functional form (see a complete benchmark review \cite{staerman2022functional} on the subject).
\end{remark}

\begin{remark}{ \sc (Calibration of extremes)} \label{rem:11} Since the $L^2$-norm brings only global information, some type of anomaly may fall through the cracks at the truncation step and this is why our algorithm has to be coupled with an non-extreme study of anomalies. If we consider $\mathcal{C}([0,1])$-regularly varying variables, a solution would be to condition extreme observations w.r.t. an other metric, continuous for the supremum norm, e.g. $l(x) = \beta \|x\|_2 + (1- \beta) \|x\|_\infty$ or $l(x) = \beta \|x\|_2 + (1- \beta) w_x(\delta)$, with $\beta \in (0,1)$ and $w_x(\delta):= \sup_{|s-t| \m \delta}|x(s)-x(t)|$, the modulus of continuity of $x$ with tolerance threshold $\delta$ (limit extreme process existence is ensured by Theorem 3 of \cite{dombry2015functional}).
\end{remark}
\subsubsection{Functional Marginal Standardization}

\begin{definition}Let $X$ be a stochastic process with sample paths in $\mathcal{C}([0,1])$ and denote by $F_X$ the cumulative distribution function of $X$ defined s.t. for all $x \in \bb{R}$ and $t\in [0,1]$
\begin{equation*}
F_X(x,t) = \bb{P}\{X(t) \m x \}.
\end{equation*}
Define the marginal transformation of $X$ for all $t \in [0,1]$ by $V(X)(t) = \frac{1}{1-F_X(X(t),t)}$.
\end{definition}


\begin{definition}Let $X$ be a stochastic process with sample paths in $L^2([0,1])$ and denote by $F_X$ the cumulative distribution function of $X$ w.r.t. the Hilbert basis $(e_i)_{i \s 1 }$ defined s.t. for all $x \in \bb{R}$ and $i\s 1$
\begin{equation*}
F_X(x,i) = \bb{P}\{\langle X,e_i \rangle \m x \}.
\end{equation*}
Define the coordinate transformation of $X$ w.r.t. the basis $(e_i)_{i \s 1 }$  for all $i \s 1$ by $\sum_{i=1}^{+\infty}V(X)(i)e_i$ where $V(X)(i) = \frac{1}{1-F_X(X,i)}$.
\end{definition}

\textcolor{red}{pas plausible car si $X \in L^2$ on a même pas $V(X) \in L^2([0,1])$}

%\begin{remark} Let $X \in L^2([0,1])$ (resp. $X \in \mathcal{C}([0,1])$). If $X$ is regularly varying then, for all Hilbert basis $(e_i)_{i \s 1}$, for all $j\s 1$, $\langle X,e_j \rangle$ is regularly varying in $\bb{R}$ (resp. for all $t \in [0,1]$, $X(t)$ is regularly varying in $\bb{R}$). In particular, with the above transformation, this condition is fulfilled.
%\end{remark}
%NB: $X \in RV_{-\alpha}(\bb{R}^d) \Leftrightarrow V(X) \in RV_{-1}(\bb{R}^d)$

\subsection{Hilbert Mixture Model}
\begin{lemma}\label{lemma:6.3}
Let $(e_j)_{j \s 1}$ be a Hilbert basis, let $d \s 1$ be an integer and let $(X_j)_{1 \m j \m d}$ be real-valued random variables. The two following statements are equivalent.
\begin{itemize}
	\item[(i)] $(X_1,...,X_d) \in RV_{-\alpha}(\bb{R}^d)$ s.t. there exist a positive sequence $(a_n)_{n \s 1}$ and a nonzero $\bb{M}_0$-measure $\mu$ s.t. $\mu_n( \cdot ):= n \bb{P}\{a_n^{-1}(X_1,...,X_d) \in \cdot\} \overset{\bb{M}_0}{\lra} \mu$;
	\item[(ii)] $\sum_{i=1}^d X_i e_i \in RV_{-\alpha}(\bb{H})$ s.t. there exist a positive sequence $(b_n)_{n \s 1}$ and a nonzero $\bb{M}_0$-measure $\Tilde{\mu}$ s.t. $\Tilde{\mu}_n( \cdot ):= n \bb{P}\{b_n^{-1}\sum_{i=1}^d X_i e_i \in \cdot\} \overset{\bb{M}_0}{\lra} \Tilde{\mu}$.
\end{itemize}
In particular, if an assertion is fulfilled, $(a_n)_{n \s 1}$ could be equal to $(b_n)_{n \s 1}$ and the following relation holds true, $\Tilde{\mu}(B) = \mu(\Psi^{-1}(B))$, where $B$ is a continuity-set, bounded away from the origin, of $\mu$ and $\Psi : (x_1,...,x_d) \in \bb{R}^d \mapsto \sum_{i = 1}^d x_i e_i \in Vect\{e_1,...,e_d\}$.
\end{lemma}

\begin{remark} Lemma \ref{lemma:6.3} is of prime order for our study and in particular for simulation experiments. It allows to simply construct regularly varying random functions in $L^2([0,1])$ given a Hilbert basis. Even though those random functions belongs in a subjacent finite dimensional space, it represents the first step of a more complicated model.
\end{remark}
The following result first appears in \cite{HL05} but it can be found in the two mentioned references in a more suitable way.
\begin{lemma}[Hilbert analogue of Lemma 3.11 in \cite{jessen2006regularly} or Proposition 7.4 in \cite{resnick2007heavy}.]
Let $X$ and $Y$ be two $\bb{H}$-random variables defined on the same probability space, independent and regularly varying such that
\begin{equation*}
n \bb{P}\{a_n^{-1}X \in \cdot \} \overset{\bb{M}_0}{\rightarrow} \mu_1, \text{ and } n \bb{P}\{a_n^{-1}Y \in \cdot \} \overset{\bb{M}_0}{\rightarrow} \mu_2.
\end{equation*}

Then, $X+Y$ is regularly varying such that
\begin{equation*}
n \bb{P}\{a_n^{-1}(X+Y) \in \cdot \} \overset{\bb{M}_0}{\rightarrow} \mu_1 + \mu_2.
\end{equation*}
\end{lemma}
\begin{proof}
One can apply mutatis-mutandis the proof of Lemma 7.2 in \cite{resnick2007heavy} in order to prove that
\begin{equation*}
n \bb{P}\{a_n^{-1}(X,Y)\in \cdot \} \overset{\bb{M}_0}{\rightarrow} \Tilde{\mu},
\end{equation*}
with $\Tilde{\mu}(dx,dy) = \mu_1(dx)\epsilon_0(dy) + \mu_2(dy)\epsilon_0(dx)$.
Since the map $SUM : (x,y) \in \bb{H}^2 \mapsto x+y \in \bb{H}$ is linear and continuous, we have that
\begin{equation*}
n \bb{P}\{a_n^{-1}(X+Y) \in \cdot \} = n \bb{P}\{a_n^{-1}SUM(X,Y)\in \cdot \} \overset{\bb{M}_0}{\rightarrow} \Tilde{\mu}\circ SUM^{-1} = \mu_1+\mu_2.
\end{equation*}
\end{proof}
\begin{proposition}
Let $(e_j)_{j \s 1}$ be a Hilbert basis and let $d \s 1$ be an integer. Let $b_1,...,b_d$ be i.i.d. Bernoulli random variables with parameter $0 < p < 1$. Let $W_1,...,W_d$ be i.i.d. regularly varying random variables in $\bb{R}_+$, s.t. $n\bb{P}\{a_n^{-1}X \in \cdot \} \overset{\bb{M}_0}{\rightarrow} \mu_j$ and let $Y_1,...,Y_d$ be i.i.d. random variables in $\bb{R}$. We assume that the $b_j$'s, the $W_j$'s and the $Y_j$'s are independent and also that $\bb{P}\{Y_1 \s x \} = o(\bb{P}\{W_1 \s x \})$. Then, the following random function
\begin{equation}
X := \sum_{i=1}^d (b_i W_i + (1-b_i)Y_i)e_i 
\end{equation}
is regularly varying in $\bb{H}$ s.t.
\begin{equation}
n \bb{P}\{ a_n^{-1}X \in B \} \nti \Tilde{\mu}_d(B),
\end{equation}
for all $B$ continuity-set of $\Tilde{\mu}_d$ bounded away from zero and with $\Tilde{\mu}_d(B):= \sum_{j=1}^{2^d} \mu_{\Omega_j}(B) \bb{P}\{ I_1 = \Omega_j\}$ and $\mu_{\Omega_j}(B):= \sum_{i \in \Omega_j} \mu_i(B)$.
\end{proposition}
\begin{proof}
Since $W_1,...,W_d$ are regularly varying and $\bb{P}\{Y_1 \s x \} = o(\bb{P}\{W_1 \s x \})$, then by adapting mutatis-mutandis Lemma 3.12 of \cite{jessen2006regularly} to the general Hilbert case, we obtain that for all part $\Omega_j$ of $\{1,...,d\}$,
\begin{equation*}
n \bb{P}\{a_n^{-1}\Big(\sum_{i \in \Omega_j} W_j e_j + \sum_{i \in \Omega_j^c} Y_j e_j \Big) \in \cdot \} \overset{\bb{M}_0}{\rightarrow} \mu_{\Omega_j},
\end{equation*}
where $\mu_{\Omega_j}$ is a Hilbert Borel measure with mass concentrated on axis $(e_j)_{j \in \Omega_j}$ and with convention, $\mu_{\Omega_j}$ is the null measure when $\Omega_j = \varnothing$. Let $B$ be a continuity-set of $\Tilde{\mu}_d$ bounded away from zero.
\begin{align*}
n \bb{P}\{a_n^{-1}X \in B \} &= \sum_{j=1}^{2^d} n \bb{P}\{a_n^{-1}X \in B \mid I_1 = \Omega_j \} \bb{P}\{I_1 = \Omega_j \} \\
&= \sum_{j=1}^{2^d} n \bb{P}\{a_n^{-1}\Big( \sum_{i \in \Omega_j} W_i e_i + \sum_{i \in \Omega_j^c} Y_i e_i \Big) \in B \} \bb{P}\{ I_1 = \Omega_j \} \\
&\nti \sum_{j=1}^{2^d} \mu_{\Omega_j}(B) \bb{P}\{ I_1 = \Omega_j\}:=\Tilde{\mu}_d(B),
\end{align*}
where $I_1:=\{ 1 \m i \m d, b_i =1 \}$ and notice that a continuity-set for $\Tilde{\mu}_d$ is then a continuity-set for each $\mu_{\Omega_j}$. The last formula of $\mu_{\Omega_j}$ follows from the Hilbert analogue of Lemma 3.11 in \cite{jessen2006regularly}.
\end{proof}
\begin{remark} Notice that for all $i \s 1$ and $r \s 1$, we have $\mu_i(\bb{B}(0,r)^c) = r^{-\alpha} \mu_1(\bb{B}(0,1)^c)$.
\end{remark}

\begin{proposition}
Let $(e_j)_{j \s 1}$ be a Hilbert basis. Let $\delta$ be an integer-valued random variable s.t. $\E [\delta ] < +\infty$ and let $(W_j)_{j \s 1}$ be an i.i.d. sequence of regularly varying random variables in $\bb{R}_+$, independent of $\delta$. Then, the following random function
\begin{equation}
X = \sum_{i=1}^\delta W_i e_i
\end{equation}
is regularly varying in $\bb{H}$ s.t.
\begin{equation*}
n \bb{P}\{ a_n^{-1} X \in B \} \nti \sum_{d=1}^{+\infty} \bb{P}\{ \delta = d \} \mu_{\{1,...,d\}}(B).
\end{equation*}
\end{proposition}
\begin{proof}
Let $B$ be a continuity-set of each $\mu_j$ bounded away from zero. Since $\mu_{\{1,...,d\}}(B) \m d \mu_1(\bb{B}(0,1)^c)$
\begin{align*}
n \bb{P}\{ a_n^{-1}X \in B \} &= \sum_{d=1}^{+\infty} \bb{P}\{\delta =d \} n \bb{P}\{ a_n^{-1}\sum_{i=1}^d W_i e_i \in B \} \\
& \nti \sum_{d=1}^{+\infty} \bb{P}\{\delta =d \} \mu_{\{1,...,d\}}(B),
\end{align*}
where the convergence follows from the dominated convergence theorem with domination $\bb{P}\{\delta =d \} n \bb{P}\{ a_n^{-1}\sum_{i=1}^d W_i e_i \in B \} \m \bb{P}\{\delta =d \}d \mu_1 (\bb{B}(0,1)^c)$ for $n$ large enough.
\end{proof}

\begin{proposition}
Let $(e_j)_{j \s 1}$ be a Hilbert basis. Let $\delta$ be an integer-valued random variable and let $(b_j)_{j \s 1}$ be i.i.d. Bernoulli random variables with parameter $0 < p < 1$. Let $(W_j)_{j \s 1}$ be an i.i.d. sequence of regularly varying random variables in $\bb{R}_+$ and let $(Y_j)_{j \s 1}$ be an i.i.d. sequence of random variables in $\bb{R}$. Assume all possible independences between the consider random variables and assume also that $\bb{P}\{Y_1 \s x \} = o(\bb{P}\{W_1 \s x \})$ and $\E [ \delta (1+p)^\delta ] < +\infty$. Then, the following random function
\begin{equation*}
X := \sum_{i=1}^\delta (b_i W_i + (1-b_i)Y_i)e_i 
\end{equation*}
is regularly varying in $\bb{H}$ s.t.
\end{proposition}
\begin{proof}
Recall that for all $d \s 1$, for all $1 \m j \m 2^d$
\begin{equation*}
n \bb{P}\{a_n^{-1}\Big( \sum_{i \in \Omega_{j,d}} W_i e_i + \sum_{i \in \Omega_{j,d}^c} Y_i e_i \Big) \in \cdot\} \overset{\bb{M}_0}{\rightarrow} \mu_{\Omega_{j,d}} = \sum_{i \in \Omega_{j,d}} \mu_i.
\end{equation*}
Let $B$ be a continuity-set of each $\mu_j$ bounded away from zero.
\begin{align*}
n \bb{P}\{a_n^{-1}X \in B \} &= \sum_{d=1}^{+\infty} n \bb{P}\{a_n^{-1}X \in B \mid \delta = d\} \bb{P}\{\delta = d \} \\
&= \sum_{d=1}^{+\infty} \sum_{j=1}^{2^d} n \bb{P}\{a_n^{-1}\Big( \sum_{i \in \Omega_{j,d}} W_i e_i + \sum_{i \in \Omega_{j,d}^c} Y_i e_i \Big) \in B\} \bb{P}\{ I_1^d = \Omega_{j,d}\} \bb{P}\{\delta = d \} \\
&\nti \sum_{d=1}^{+\infty} \sum_{j=1}^{2^d} \mu_{\Omega_{j,d}}(B) \bb{P}\{I_1^d = \Omega_{j,d}\} \bb{P}\{ \delta = d \},
\end{align*}
where the convergence follows from the dominated convergence theorem since
\begin{equation*}
\sum_{j=1}^{2^d} n \bb{P}\{a_n^{-1}\Big( \sum_{i \in \Omega_{j,d}} W_i e_i + \sum_{i \in \Omega_{j,d}^c} Y_i e_i \Big) \in B\} \bb{P}\{ I_1^d = \Omega_{j,d}\} \bb{P}\{\delta = d \} \m \mu_1( \bb{B}(0,1)^c) d(1+p)^d \bb{P}\{\delta = d \}
\end{equation*}
for $n$ large enough.
\end{proof}

\begin{remark}
The condition "$\E [ \delta (1+p)^\delta ] < \infty$" is actually not at all restrictive. All finite discrete random variables fulfilled this condition and if one thinks about the most usual counting process, namely the Poisson process, $\delta$ following a Poisson distribution also satisfies the requirement.
Finiteness of the first moment of $\delta$ is an usual assumption when dealing with random sums to avoid the possibility of a sum with an infinite number of terms. However, Hilbert basis decompositions are not traditional series and then, under additional assumptions, it could be natural to consider Hilbert basis decompositions with an infinite number of terms or at least with $\delta$ terms s.t. $\E [\delta] = + \infty$.
\end{remark}



==> ContinuousRVimpliesHRV.tex <==



==> GARCH.tex <==
\subsection{Global extremal behavior of COGARCH(1,1) process}

The continuous-time GARCH model was introduced in \cite{kluppelberg2004continuous}, known as \emph{COGARCH} model. In the following, we only deal with the COGARCH(1,1) model which is abusively called the COGARCH model (see \cite{brockwell2006continuous} for a general definition of a COGARCH(p,q) model). The COGARCH model is defined as follow.

Let $(L_t)_{t \s 0}$ be a Lévy process with jumps $\Delta L_t = L_t - L_{t-}$ and characteristic triplet $(\gamma, \sigma^2, \Pi_L)$, \ie the characteristic function of $L$, denoted by $\varphi_L$, is given by
\begin{align*}
\varphi_L(\theta)(t) &:= \E [ \exp(i\theta L_t) ] \\
&=\exp \Big( t( \gamma i \theta - \frac{\sigma^2 \theta^2}{2} + \int_{\bb{R}\backslash \{0\}}(\exp(i\theta x) -1 -i \theta x \1\{|x|<1\}) \Pi_L(dx))]\Big),
\end{align*}
with $\Pi_L$ Lévy measure of $L$ s.t.
\begin{equation*}
\int_{\bb{R}\backslash \{0\}} \min(0,x^2) \Pi_L(dx) < \infty.
\end{equation*}
The COGARCH process $(G_t)_{t \s 0}$ is defined via the following stochastic differential equation (SDE)
\begin{equation}\label{eq:COGARCH}
dG_t = \sigma_t dL_t, t\s 0,
\end{equation}
where $(\sigma_t)_{t \s 0}$ is the volatility process fulfilling
\begin{equation}\label{eq:vol_COGARCH}
d\sigma_{t+}^2 = (\beta - \eta \sigma_t^2)dt + \lambda \mathrm{e}^\eta\sigma_t^2 d[L,L]_t,
\end{equation}
with constants $\beta > 0, \eta > 0, \lambda \s 0$ and $[L,L]_t$ given by
\begin{equation*}
[L, L]_t \quad:=\sum_{0<s \leq t}\left(\Delta L_s\right)^2, t\s 0, 
\end{equation*}
with $L_{0-}:=0$.

We refer to \cite{kluppelberg2004continuous} for technical details of presented results about COGARCH process.

Define the auxiliary Lévy process $(X_t)_{t \s 0}$
\begin{equation}
X_t=\eta t-\sum_{0<s \leq t} \ln \left(1+\lambda \mathrm{e}^\eta\left(\Delta L_s\right)^2\right), \quad t \geq 0,
\end{equation}
then a solution of the SDE \eqref{eq:vol_COGARCH} can be displayed in terms of $(X_t)_{t \s 0}$
\begin{equation} \label{eq:vol_sol}
\sigma^2_t=\left(\beta \int_0^t \mathrm{e}^{X_s} d s+\sigma^2_0\right) \mathrm{e}^{-X_{t-}}, \quad t \geq 0.
\end{equation}
Moreover, there exists a stationary version of \ref{eq:vol_sol} under the necessary condition that
\begin{equation*}
\int_{\mathbb{R}} \ln \left(1+\lambda \mathrm{e}^\eta y^2\right) \Pi_L(d y)<\eta,
\end{equation*}
and is then given by the equation \eqref{eq:vol_sol} for $\sigma_0^2 \overset{d}{=} \beta \int_0^\infty  \mathrm{e}^{-X_{t}}dt$.

A central object to study the extremal behavior of the volatility process $(\sigma_t^2)_{t \s 0}$, and more precisely to determine the index of regular variation of the process, is the Laplace transform of the process $(X_t)_{t \s 0}$, $\E [\mathrm{e}^{-sX_{t}}] = \mathrm{e}^{t\phi(s)}$, and in particular the Laplace exponent
\begin{equation}
\Psi(s)=-\eta s+\int_{\mathbb{R}}\left(\left(1+\lambda \mathrm{e}^\eta y^2\right)^s-1\right) \Pi_L(d y), \quad s \geq 0.
\end{equation}
The importance of $\Psi$ ensues from Theorem 4 in \cite{fasen2006extremal} which is recalled for convenience here.

\begin{theorem}[Theorem 4 in \cite{fasen2006extremal}]\label{thm:RV_GARCH}
Suppose there exists some $\alpha>0$ such that
\begin{equation}
\mathbb{E}\left|L_1\right|^{2 \alpha} \ln ^{+}\left|L_1\right|<\infty \quad \text { and } \quad \Psi(\alpha)=0.
\end{equation}
Let $\sigma^2$ be a stationary version of the volatility process given by \eqref{eq:vol_sol}. Then for some constant $C>0$ we have
\begin{equation}
\lim _{x \rightarrow \infty} x^\alpha \mathbb{P}\left(\sigma^2_0>x\right)=C.
\end{equation}
\end{theorem}
In the same way as authors in \cite{fasen2006extremal}, in order to derive explicit formulas for extremal quantities of the volatility process, we will restrict our study to a specific driving Lévy process $L$. Hence, in the following, $L$ will be a compound Poisson process given by $L_t = \sum_{i=1}^{N_t}\xi_i$, with $N = \{N_t, t \s 1\}$ is a counting Poisson process with intensity parameter $\mu$ and $\xi_j$ the value at the $j$-th arrival (\textcolor{red}{à determiner}). We denote by $(\Gamma_k)_{k \in \bb{N}}$ the sequence of arrival times (with the convention $\Gamma_0 := 0$) and recall that inter-arrival times $\Gamma_{k+1}-\Gamma_k$ are independent and exponentially distributed with parameter $\mu$. With this framework, authors in \cite{kabanov2006continuous} proved that the volatility process is exactly given by the equations
\begin{equation}
\sigma^2_{\Gamma_k+}-\sigma^2_{\Gamma_k}=\lambda \mathrm{e}^\eta \sigma^2_{\Gamma_k} \xi_k^2, \quad k \in \mathbb{N},
\end{equation}
and,
\begin{equation}
\sigma^2_t=\frac{\beta}{\eta}+\left(\sigma^2_{\Gamma_k+}-\frac{\beta}{\eta}\right) \mathrm{e}^{-\left(t-\Gamma_k\right) \eta}, \quad t \in\left(\Gamma_k, \Gamma_{k+1}\right].
\end{equation}
Finally, if we set $\Tilde{\sigma}^2_k:=\sigma^2_{\Gamma_k+}$, authors in \cite{fasen2006extremal} have shown the exact analogue of Theorem \ref{thm:RV_GARCH} for the sequence $(\Tilde{\sigma}^2_k)_{k \in \bb{N}}$ with an explicit constant $C$. We state Theorem 5 of \cite{fasen2006extremal} for convenience here.
\begin{theorem}[Theorem 5 in \cite{fasen2006extremal}]\label{thm:RV_GARCH_POISSON}
Suppose there exists some $\alpha>0$ such that
\begin{equation}
\mathbb{E}\left|L_1\right|^{2 \alpha} \ln ^{+}\left|L_1\right|<\infty \quad \text { and } \quad \Psi(\alpha)=0
\end{equation}
Then a stationary solution $\left(\sigma^2_k\right)_{k \in \mathbb{N}}$ of (4.61) exists. Its marginal stationary distribution, denoted by $\tilde{V}_0$, is the unique solution of the random fix point equation
\begin{equation*}
\tilde{\sigma}^2_0 \stackrel{d}{=} \widetilde{A} \tilde{\sigma}^2_0+\widetilde{B}
\end{equation*}
where $\tilde{A} \overset{d}{=}\mathrm{e}^{-X_{\Gamma_1}}$ and $\tilde{B}\overset{d}{=}\beta\mathrm{e}^{-X_{\Gamma_1}}\int_0^{\Gamma_1}\mathrm{e}^{X_s}ds$ are independent of $L$ and $\tilde{\sigma}^2_0$. Furthermore,
\begin{equation}
\mathbb{P}\left(\tilde{\sigma}^2_0>x\right) \sim \widetilde{C} x^{-\alpha}, \quad x \rightarrow \infty
\end{equation}
where
\begin{equation}
\widetilde{C}=\frac{\mathbb{E}\left[\left(\tilde{A} \tilde{\sigma}^2_0+\widetilde{B}\right)^\alpha-\left(\widetilde{A} \tilde{\sigma}^2_0\right)^\alpha\right]}{\alpha \mathbb{E}|\widetilde{A}|^\alpha \ln ^{+}|\widetilde{A}|}>0
\end{equation}
\end{theorem}



To the best of our knowledge, only the extremal behavior of marginal distributions of the volatility process (and the COGARCH process) has been investigated. Relying on those properties we aim to prove global functional regular variation conditions of the volatility process. Since the volatility process $(\sigma^2)_{t\s 0}$ is a càdlàg process, the regular variation in the space of continuous function cannot be investigated. We then study the regular variation in $L^2([0,1])$ by considering the volatility process restricted to the interval $[0,1]$.

Define the stopping time $\mathcal{J}:= \inf \{ j \in \bb{N}, \Gamma_{j} \m 1, \Gamma_{j+1}>1 \}$. Then, the stationary volatility process can be decomposed on $[0,1]$ as follow
\begin{equation}
\sigma^2_t = \frac{\beta}{\eta}+ \sum_{i=0}^{\mathcal{J}-1}\sigma^2_{i,t}  + \bar{\sigma}^2_{\mathcal{J},t},
\end{equation}
where $\sigma^2_{j,t}:= \left(\Tilde{\sigma}^2_j-\frac{\beta}{\eta}\right) \mathrm{e}^{\Gamma_j \eta}g_\eta(t)\1\{t \in (\Gamma_j, \Gamma_{j+1} ]\}$ and $\bar{\sigma}^2_{\mathcal{J},t}=\left(\Tilde{\sigma}^2_\mathcal{J}-\frac{\beta}{\eta}\right) \mathrm{e}^{\Gamma_\mathcal{J}\eta}g_\eta(t)\1\{t \in (\Gamma_\mathcal{J},1]\}$  for $j \in \bb{N}$ and with $g_\eta(t)= \mathrm{e}^{-t \eta}$.

\begin{proposition}\textcolor{red}{FAUX}
Let $j< \mathcal{J}$. Then $(\sigma^2_{j,t})_{t \in [0,1]} \in RV_{-\alpha}(L^2([0,1]))$, with $\alpha$ as in Theorem \ref{thm:RV_GARCH_POISSON} and s.t.
\begin{equation}
\mathcal{L}\Big(\frac{\sigma^2_{j,\cdot}}{\|\sigma^2_{j,\cdot}\|_2} \mid \|\sigma^2_{j,\cdot}\|_2\s r \Big) \underset{r \rightarrow +\infty}{\longrightarrow} \mathcal{L}(\Theta_j),
\end{equation}
with 
\begin{equation}
\bb{P}\{\Theta_j \in A \} = \frac{\E \Big[ \Big( \frac{1-g_\eta(2(\Gamma_{j+1}-\Gamma_j))}{2\eta}\Big)^{\alpha/2} \1\Big\{\frac{g_\eta(\cdot-\Gamma_j) \1\{(\Gamma_j,\Gamma_{j+1})\}}{\|g_\eta(\cdot-\Gamma_j) \1\{(\Gamma_j,\Gamma_{j+1})\}\|_2} \in A \Big\}\Big]}{\E \Big[ \Big( \frac{1-g_\eta(2(\Gamma_{j+1}-\Gamma_j))}{2\eta}\Big)^{\alpha/2}\Big]}.
\end{equation}

%\begin{equation}
%\mathcal{L}\Big(\frac{\sigma^2_{\mathcal{J},\cdot}}{\|\sigma^2_{\mathcal{J},\cdot}\|_2} \mid \|\sigma^2_{\mathcal{J},\cdot}\|_2\s r \Big) \underset{r \rightarrow +\infty}{\longrightarrow} \mathcal{L}\Big(\frac{\eta g_\eta \1\{(\Gamma_\mathcal{J}, 1]\} }{g_\eta(\Gamma_\mathcal{J})-g_\eta(1)}\Big).
%\end{equation}
\end{proposition}
\begin{proof}
We will prove the characterization \ref{thm:RVH2} of Theorem \ref{thm:RVH} to obtain the regular variation property and then explicit formulas of limit angular processes will straightforwardly ensue. 

Let $j<\mathcal{J}$ \textcolor{red}{on ne peut pas considérer un tel entier il faut conditionner dans les probas par rapport à $\mathcal{J}$}. Since $\tilde{\sigma}^2_j \in RV_{-\alpha}$, denote by $\mu$ the nonzero Radon measure finite and $(b_n)_{n \s 1}$ the regularly varying positive sequence s.t.
\begin{equation*}
b_n \bb{P}\{n^{-1}\tilde{\sigma}^2_j \in \cdot \} \overset{v}{\rightarrow} \tilde{\mu}.
\end{equation*}
First, notice that $\|\sigma^2_{j,\cdot}\|_2 = (\tilde{\sigma}_j^2 - \frac{\beta}{\eta})\sqrt{\frac{1-\exp ( - 2\eta(\Gamma_{j+1}-\Gamma_j))}{2\eta}}$ is regularly varying with index $\alpha$ since $\tilde{\sigma}_j^2$ is regularly varying with index $\alpha$, $\tilde{\sigma}_j^2$ is independent from $\Gamma_{j+1}-\Gamma_j$ \textcolor{red}{mais dependent de $\Gamma_j$} and, following Lemma 4.2 from \cite{jessen2006regularly}, we know that
\begin{equation*}
\bb{P}\{\|\sigma^2_{j,\cdot}\|_2 \s r \} \underset{x \rightarrow + \infty}{\sim} \E\Big[\Big(\frac{1-\exp ( - 2\eta(\Gamma_{j+1}-\Gamma_j))}{2\eta}\Big)^{\alpha/2} \Big] \bb{P}\{ \|\tilde{\sigma}^2_j\|_2 \s r \}. \textcolor{red}{vrai}
\end{equation*}



Let $B \in \mathcal{B}(L^2([0,1]))$ be a $\mu$-continuity set. Following Lemma 4.6 of \cite{jessen2006regularly}, we have 
\begin{align*}
b_n \bb{P}\{n^{-1} \sigma^2_{j,\cdot} \in B \} &= \E [b_n \bb{P}\{n^{-1} \sigma^2_{j,\cdot} \in B  \mid \Gamma_j, \Gamma_{j+1}\} ] \\
&=\E \Big[ b_n \bb{P}\{n^{-1} (\tilde{\sigma}^2_j-\frac{\beta}{\eta}) \in B_\eta(\Gamma_j,\Gamma_{j+1}) | \Gamma_j, \Gamma_{j+1} \} \Big] \\
&\nti \E [ \tilde{\mu}(B_\eta(\Gamma_j,\Gamma_{j+1})) ] \\
&=\E [ \tilde{\mu}(\{ x>0, x g_\eta(\cdot - \Gamma_j) \1\{(\Gamma_j, \Gamma_{j+1}]\} \in B \}) ]:=\mu_j,\textcolor{red}{faux}
\end{align*}
with $B_\eta(\Gamma_j,\Gamma_{j+1})=\{x > 0, x \mathrm{e}^{\Gamma_j \eta}g_\eta\1\{(\Gamma_j, \Gamma_{j+1} ]\} \in B \}$ and where the Pratt's lemma is used in the limit relation (see \cite{pratt1960interchanging}).
Finally, by simple calculus, we obtain
\begin{equation}
\bb{P}\Big\{ \frac{\tilde{\sigma}_{j,\cdot}}{\|\tilde{\sigma}_{j,\cdot}\|_2} \in A \Big| \|\tilde{\sigma}_{j,\cdot}\|_2 \s r \Big\}\underset{r \rightarrow +\infty}{\longrightarrow} \frac{\E \Big[ \Big( \frac{1-g_\eta(2(\Gamma_{j+1}-\Gamma_j))}{2\eta}\Big)^{\alpha/2} \1\Big\{\frac{g_\eta(\cdot-\Gamma_j) \1\{(\Gamma_j,\Gamma_{j+1})\}}{\|g_\eta(\cdot-\Gamma_j) \1\{(\Gamma_j,\Gamma_{j+1})\}\|_2} \in A \Big\}\Big]}{\E \Big[ \Big( \frac{1-g_\eta(2(\Gamma_{j+1}-\Gamma_j))}{2\eta}\Big)^{\alpha/2}\Big]}.
\end{equation}
\end{proof}
\begin{remark} If one consider deterministic jump arrival times, notice that the distribution of the angular limit process between jumps is given by the Dirac measure at function $\frac{g_\eta(\cdot-\Gamma_j) \1\{(\Gamma_j,\Gamma_{j+1})\}}{\|g_\eta(\cdot-\Gamma_j) \1\{(\Gamma_j,\Gamma_{j+1})\}\|_2}$. \textcolor{red}{vrai}
\end{remark}
\begin{theorem}
The volatility process over $[0,1]$, $(\sigma^2_t)_{t\in [0,1]} \in RV_{-\alpha}(L^2([0,1]))$, with $\alpha$ as in Theorem \ref{thm:RV_GARCH_POISSON} and s.t. \textcolor{red}{à réécrire}
\begin{equation} 
\mathcal{L}\Big( \frac{\sigma^2}{\|\sigma^2\|_2} \mid \|\sigma^2\|_2 \s r\Big) \underset{r \rightarrow +\infty}{\longrightarrow}
\end{equation}
% \mathcal{L}\Big(\frac{\sum_{i=1}^{\mathcal{J}-1}g_\eta(\cdot-\Gamma_i)\1\{(\Gamma_i, \Gamma_{i+1}]\}+g_\eta(\cdot-\Gamma_\mathcal{J})\1\{(\Gamma_\mathcal{J}, 1]\}}{\frac{1}{\eta}\big(\sum_{i=1}^{\mathcal{K}-1}(1-\mathrm{e}^{-(\Gamma_{i+1}-\Gamma_i)\eta})+(1-\mathrm{e}^{-(1-\Gamma_\mathcal{J})})\big)}\Big) .
\end{theorem}
\begin{proof}
We will use Theorem \ref{thm:thmRVH} in order to prove that $\sigma^2$ is regularly varying in $L^2([0,1])$. Recall that three properties have to be investigated:
\begin{itemize}
\item[(1)] $\|\sigma^2\|_2$ is regularly varying in $\bb{R}$;
\item[(2)] $\exists \Theta_\infty \in \bb{S}(L^2([0,1])), \forall j \in \bb{N}^*, \E [\Big(\frac{\langle \sigma^2,e_n \rangle}{\|\sigma^2\|}\Big)^2 \mid \|\sigma^2\| \s t ] \tti \E[\langle  \Theta_\infty, e_n \rangle^2]$;
\item[(3)] $\exists \Theta_\infty \in \bb{S}(L^2([0,1])), \forall h \in L^2([0,1]), \mathcal{L}\Big(\langle \frac{\sigma^2}{\|\sigma^2\|},h \rangle \mid \|\sigma^2\| \s t \Big) \tti \mathcal{L}( \langle \Theta_\infty, h \rangle ).$
\end{itemize}
\end{proof}

==> Notations.tex <==
\begin{itemize}
	\item $(\bb{H}, \langle \cdot , \cdot \rangle)$ a separable Hilbert space with orthonormal Hilbert basis $(e_i)_{i\s 1}$;
	\item $\bb{H}_0 := \bb{H} \backslash \{0\}$;
	\item $(HS(\bb{H}),\langle \cdot , \cdot \rangle_{HS})$ the separable Hilbert space of Hilbert-Schmidt operators of $\bb{H}$;
		\item $\| \cdot \|_{HS}$ the norm associated with $\langle \cdot , \cdot \rangle_{HS}$;
	\item $\| \cdot \|$ the norm associated with $\langle \cdot , \cdot \rangle$;
	\item $\bb{S}(\bb{H})$ the unit sphere of $\bb{H}$ for $\| \cdot \|$
	\item $\Pi_{t_1,...,t_k}$ orthogonal projection onto $span\{e_{t_1},...,e_{t_d}\}$ and if no confusion is possible $\Pi_d := \Pi_{1,...,d}$
	\item $B(0,r)$ ball of radius $r$ in $\bb{H}$ for $\| \cdot \|$
	\item $RV_{-\alpha}(\bb{H})$ set of regularly varying elements of $\bb{H}$ with index $-\alpha$
	\item $(\E , \mathcal{E},\mu)$ a measure space
	\item $(\Omega, \mathcal{F},\bb{P})$ a probability space
	\item $\mathcal{C}^0_b(\bb{H})$ space of continuous and bounded functions of $\bb{H}$
	\item $\bb{D}([0,1])$ space of càdlàg functions
	\item $\tilde{\mathcal{C}}_b^0(\bb{H})$ space of continuous and bounded function of $\bb{H}$ which disappear on a neighborhood of the origin
	\item $\forall h_1,h_2 \in \bb{H}$, $h_1 \otimes h_2 := \langle h_1, \cdot \rangle h_2 \in HS(\bb{H})$
	\item $\Theta_t \overset{d}{=} X/\|X\| | \{\|X\| > t \}$
	\item $\Theta_\infty$ the limit distribution of $\Theta_t$
	\item $C_\infty := \E [\Theta_\infty \otimes \Theta_\infty ]$ with ordered eigenvalues $\lambda_\infty^1 \s \lambda_\infty^2 \s ...$
	\item $C_t := \E [\Theta_t \otimes \Theta_t ]$ with ordered eigenvalues $\lambda_t^1 \s \lambda_t^2 \s ...$
	\item $\hat{C}_t := \frac{1}{\sum_{k=1}^n \1\{\|X_k\| \s t \}}\sum_{i=1}^n \theta (X_i) \otimes \theta (X_i) \1\{\|X_i\| \s t \}$ with random eigenvalues $\hat{\lambda}_1,\hat{\lambda}_2,...$
	\item $\overline{C}_t := \frac{1}{\bb{P}(\|X\|>t)}\sum_{i=1}^n \theta (X_i) \otimes \theta (X_i) \1\{\|X_i\| \s t \}$
	\item $\theta (x) = \frac{x}{\|x\|_\bb{H}}$
	\item $\theta_t (x) = \frac{x}{\|x\|_\bb{H}}\1\{\|x\|\s t \}$ (different from $\Theta_t$ which defines the conditional law)
	\item $R_\infty(V) := \bb{E}[\| \Pi_{V^\bot} (\Theta_\infty) \|^2 ]$ with $V_\infty = \argmin_{V \subset \bb{H} : dim(V)=p} R_\infty(V) =0$.
	\item $R_t(V) := \bb{E}[\| \Pi_{V^\bot} (\Theta_t) \|^2 ]$ with $V_t^p = \argmin_{V \subset \bb{H} : dim(V)=p} R_t(V)$
\newpage
\end{itemize}

==> Proofcontreex.tex <==
Let $X \in \mb{H}$ be a random variable in the Hilbert space $\mb{H}$. Let $\{e_i \}$ be a orthonormal hilbertian basis of $\mb{H}$. For all $k \in \mb{N}$, for all $t_1,...,t_k \in \mb{N}$, denote by $\Pi_{t_1,...,t_k}:\mb{H} \rightarrow \mb{H}$ the projection onto $span\{e_{t_1},...,e_{t_k} \}$. For the sake of brevity, $\Pi_{1,...,d}$ will be abbreviated by $\Pi_d$. In the following, a counter example of the below statement will be proved:
\begin{center}
"$\forall k \in \mb{N}, t_1,...,t_k \in \mb{N},  \Pi_{t_1,...,t_k}X \in RV(\mb{H})$ and $\|X\| \in RV(\mb{R})$ \underline{imply that} $X \in RV(\mb{H})$."
\end{center}
\section{Proof}
Lets consider $X := R \Theta \in \mb{H}$ with
\begin{itemize}
	\item $R \sim Pareto(\alpha)$ on $[1, +\infty [$, \emph{i.e.} $\forall t \s 1, \mb{P}(R \s t) = t^{-\alpha}$
	\item we define the law of $\Theta$ conditionally to $R$ by
	$$\mathcal{L}(\Theta | R = r) = \frac{1}{\floor{r}}\sum_{i=1}^{\floor{r}} \delta_{e_i}$$
	thus, $\Theta | R = r$ is uniformly distributed over the first $\floor{r}$ vectors of basis.
\end{itemize}
In the following, we will prove:
\begin{enumerate}
	\item $\|X\| \in RV_{-\alpha}(\mb{R})$
	\item $\forall k \in \mb{N}, t_1,...,t_k \in \mb{N},  \Pi_{t_1,...,t_k}X \in RV_{-(\alpha +1)}(\mb{H})$
	\item $X \notin RV(\mb{H})$
\end{enumerate}
\begin{remark}Notice that indexes of regular variation of $\|X\|$ and finite-dimensional projections are different.
\end{remark}
\begin{enumerate}
	\item the property follows from $\|X\| = R \in RV_{-\alpha}(\mb{R})$
	\item Notice that we can only consider the projections onto the first vectors of basis, otherwise, we can reorder vectors of the basis. Let $d \in \mb{N}$. Set $\Theta_d = \frac{\Pi_dX}{\|\Pi_dX\|}$ and $R_d = \| \Pi_d X\|$. First, we show that $R_d \in RV_{-(\alpha+1)}(\mb{R})$. Let $t > d$.
\begin{align}
\mb{P}(R_d > t) &= \mb{P}(\Theta \in \{e_1,...,e_d\}, R > t) \nonumber \\
&= \mb{E}\bigg( \mb{P}(\Theta\in \{e_1,...,e_d\}, R > t | R)\bigg) \nonumber \\
&= \mb{E}\bigg(\1_{\{R > t \}} \frac{d}{\floor{R}}\bigg) \nonumber \\
&= \int_t^{+\infty} \frac{d}{\floor{r}}\alpha r^{-(\alpha+1)}dr \nonumber
\end{align}
Notice that $r \mapsto \frac{d}{\floor{r}}\alpha r^{-(\alpha+1)} \in RV_{- (\alpha +2 )}(\mb{R})$ (easy-to-prove by using the classical inequation which defines the integer part). Hence, $R_d \in RV_{- (\alpha +1 )}(\mb{R})$ follows from Karamata's theorem (p.25 in \cite{resnick2007heavy}).

Then, we have to prove that $\mathcal{L}(\Theta_d | R_d \s t )$ converges when $t$ tends to infinity. Since $\Theta$ knowing $R$ is uniformly distributed, we have for all $t>d$, and for every $i \m d$
$$\mb{P}(\Theta_d = e_i | R_d \s t ) = \mb{P}(\Theta_d = e_1 | R_d \s t )$$
Hence, $\mathcal{L}(\Theta_d | R_d \s t )$ is uniformly distributed over $\{e_1,...,e_d\}$ when $t$ is large enough.

Finally, for all $d \in \mb{N}$, $\Pi_dX$ is regularly varying in $\mb{H}$ with tail index $-(\alpha+1)$ (see proposition 2.1 in \cite{meinguet2010regularly} for a characterisation of regular variation in a Banach space).

	\item To conclude the proof, we will show that $X \notin RV(\mb{H})$. Since $\|X\| \in RV_{-\alpha}(\mb{R})$, we have to prove that $\mathcal{L}(\frac{X}{\|X\|}|\|X\| \s t)$ does not converge when $t$ tends to infinity. Thanks to theorem 1.8.4. in \cite{vaart1997weak}, it is enough to show that the asymptotically finite-dimensional condition does not hold for a sequence of random variable with respective law $\mathcal{L}(\frac{X}{\|X\|}|\|X\| \s n)$, \emph{i.e.} it is enough to show that
	$$\exists \delta,\varepsilon >0, \forall d \in \mb{N}^*, \limsup_n \mb{P}\bigg( \sum_{j> d } \langle \Theta, e_j \rangle^2 \s \delta \bigg| R \s n \bigg) \s \varepsilon$$
Let $\delta > 0, \varepsilon \in ]0,1[$ and let $n>d$.
\begin{align}
 &\mb{P}\bigg( \sum_{j> d } \langle \Theta, e_j \rangle^2 \s \delta \bigg| R \s n \bigg) \nonumber \\
= &\mb{P}( \Theta \notin \{ e_1,...,e_d\} | R \s n ) \nonumber \\
= &\E \bigg( 1 - \mb{P}(\Theta \in \{e_1,...,e_d \} | R \s n ) \bigg| R \s n \bigg) \nonumber \\
= &\E \bigg( 1 - \frac{d}{\floor{R}} \bigg| R \s n \bigg) \nonumber \\
\s &1 - \frac{d}{n} \nti 1 \s \varepsilon \nonumber
\end{align}
Hence, the asymptotic finite-dimensional condition does not hold and $X \notin RV(\mb{H})$.
\end{enumerate}

\section{With the same tail index}
Here, a second counter-example is given but the tail index of $\|X\|$ will be equal to the tail of $\|\Pi_dX\|$. The proof is very similar to the first one.

Once again, lets consider $X:= R \Theta \in \mb{H}$ with
\begin{itemize}
		\item $R \sim Pareto(\alpha)$ on $[1, +\infty [$, \emph{i.e.} $\forall t \s 1, \mb{P}(R \s t) = t^{-\alpha}$
	\item we define the law of $\Theta$ conditionally to $R$ by
	$$\mathcal{L}(\Theta | R = r) = \frac{1}{\sum_{k=1}^{\floor{r}} \frac{1}{k}}\sum_{i=1}^{\floor{r}} \frac{1}{i} \delta_{e_i}$$
	\emph{i.e.} $\Theta \in \{e_1,e_2,...\}$ and $\forall r \s 1, \forall i \in \mb{N}^*, i\m r, \mb{P}(\Theta = e_i | R = r) = \frac{1/i}{\sum_{k=1}^{\floor{r}} \frac{1}{k}}$
\end{itemize}

Notice that $r \mapsto \sum_{k=1}^{\floor{r}} \frac{1}{k}$ is slowly varying since $\sum_{k=1}^{\floor{r}} \frac{1}{k} \underset{r \rightarrow \infty}{\sim} \log r$.

In the following, we will prove:
\begin{enumerate}
	\item $\|X\| \in RV_{-\alpha}(\mb{R})$
	\item $\forall k \in \mb{N}, t_1,...,t_k \in \mb{N},  \Pi_{t_1,...,t_k}X \in RV_{-\alpha}(\mb{H})$
	\item $X \notin RV(\mb{H})$
\end{enumerate}
\begin{enumerate}
	\item $\|X\| = R \in RV_{-\alpha}(\mb{R})$
	\item Notice that we can only consider the projections onto the first vectors of basis, otherwise, we can reorder vectors of the basis. Let $d \in \mb{N}$. Set $\Theta_d = \frac{\Pi_dX}{\|\Pi_dX\|}$ and $R_d = \| \Pi_d X\|$. First, we show that $R_d \in RV_{-\alpha}(\mb{R})$. Let $t > d$.
	\begin{align}
	\mb{P}(R_d > t) &= \mb{P}(R_d \s t, R \s t) \nonumber \\
	&= \mb{P}( \Theta \in \{ e_1,...,e_d \} , R \s t) \nonumber \\
	&= \E \bigg( \1_{R \s t } \mb{P}(\Theta \in \{ e_1,...,e_d \} |R) \bigg) \nonumber \\
	&= \E \bigg( \1_{R \s t } \frac{\sum_{i=1}^{d}1/i}{\sum_{i=1}^{\floor{R}}1/i} \bigg) \nonumber \\
	&= \sum_{i=1}^{d}1/i \int_t^\infty \frac{\alpha r^{-(\alpha+1)}}{\sum_{i=1}^{\floor{r}}1/i} dr \nonumber
	\end{align}
	Notice that $r \mapsto \sum_{i=1}^{d}\frac{1}{i}\frac{\alpha r^{-(\alpha+1)}}{\sum_{i=1}^{\floor{r}}1/i} \in RV_{- (\alpha +1 )}(\mb{R})$. Hence, $R_d \in RV_{- \alpha}(\mb{R})$ follows from Karamata's theorem (p.25 in \cite{resnick2007heavy}).
	
	Then, we have to prove that $\mathcal{L}(\Theta_d | R_d \s t)$ converges when $t$ tends to infinity. First, $\Theta_d \in \{e_1,...,e_d\}$. Let $i \in \mb{N}^*, i \m d$ and let $t \s d$.
	\begin{align}
		\mb{P}(\Theta_d = e_i | R_d \s t) &= \mb{P}(\Theta = e_i | R_d \s t) \nonumber \\
		&= \frac{\mb{P}(\Theta = e_i , R_d \s t)}{\mb{P}(R_d \s t)} \nonumber \\
		&= \frac{\mb{P}(\Theta = e_i , R \s t)}{\mb{P}(R_d \s t)} \nonumber \\
		&= \frac{\E\bigg(\1_{R \s t } \frac{1/i}{\sum_{k=1}^{\floor{R}}1/k}\bigg)}{\E\bigg(\1_{R \s t } \frac{\sum_{k=1}^d 1/k}{\sum_{k=1}^{\floor{R}}1/k}\bigg)} \nonumber \\
		&= \frac{1/i}{\sum_{k=1}^{d}1/k} \nonumber
	\end{align}
Hence, when $t$ is large enough, $\mathcal{L}(\Theta_d | R_d \s t) = \frac{1}{\sum_{k=1}^{d}1/k} \sum_{i=1}^d \frac{1}{i} \delta_{e_i}$.
Finally, for all $d \in \mb{N}$, $\Pi_dX$ is regularly varying in $\mb{H}$ with tail index $-\alpha$ (see proposition 2.1 in \cite{meinguet2010regularly} for a characterisation of regular variation in a Banach space).

	\item To conclude the proof, we will show that $X \notin RV(\mb{H})$. Since $\|X\| \in RV_{-\alpha}(\mb{R})$, we have to prove that $\mathcal{L}(\frac{X}{\|X\|}|\|X\| \s t)$ does not converge when $t$ tends to infinity. Thanks to theorem 1.8.4. in \cite{vaart1997weak}, it is enough to show that the asymptotically finite-dimensional condition does not hold for a sequence of random variable with respective law $\mathcal{L}(\frac{X}{\|X\|}|\|X\| \s n)$, \emph{i.e.} it is enough to show that
	$$\exists \delta,\varepsilon >0, \forall d \in \mb{N}^*, \limsup_n \mb{P}\bigg( \sum_{j> d } \langle \Theta, e_j \rangle^2 \s \delta \bigg| R \s n \bigg) \s \varepsilon$$
Let $\delta > 0, \varepsilon \in ]0,1[$ and let $n>d$.
\begin{align}
 &\mb{P}\bigg( \sum_{j> d } \langle \Theta, e_j \rangle^2 \s \delta \bigg| R \s n \bigg) \nonumber \\
= &\frac{\mb{P}( \Theta \notin \{ e_1,...,e_d\} , R \s n )}{\mb{P}(R \s n)} \nonumber \\
= &\frac{\E\bigg(\mb{P}( \Theta \notin \{ e_1,...,e_d\} , R \s n | R) \bigg)}{\mb{P}(R \s n)} \nonumber \\
= &\frac{\E\bigg(\1_{R \s n}(1-\mb{P}( \Theta \in \{ e_1,...,e_d\} | R)) \bigg)}{\mb{P}(R \s n)} \nonumber \\
= &\frac{\E\bigg(\1_{R \s n}\big(1-\frac{\sum_{i=1}^d 1/i}{\sum_{i=1}^{\floor{R}} 1/i}\big) \bigg)}{\mb{P}(R \s n)} \nonumber \\
= &\E \bigg( 1 - \frac{\sum_{i=1}^d 1/i}{\sum_{i=1}^{\floor{R}}1/i} \ \bigg| R \s n \bigg) \nonumber \\
\s &1 - \frac{\sum_{i=1}^d 1/i}{\sum_{i=1}^{n}1/i} \nti 1 \s \varepsilon \nonumber 
\end{align}
Hence, the asymptotic finite-dimensional condition does not hold and $X \notin RV(\mb{H})$.
\end{enumerate}


==> ProofsStatsProba.tex <==
\begin{proof}
The first step is to show that $C_t$ converges towards $C_\infty$ in some sense. A convergence in operator norm would be sufficient but we will show a convergence in Hilbert-Schmidt norm which is stronger and easier to handle.
\begin{lemma}
Under aforementioned assumptions, we have
$$\|C_t - C_\infty \|_{HS(\mb{H})} \tti 0$$
\end{lemma}

We conclude 
\begin{lemma}Let $A$ be a Hilbert-Schmidt operator. Then, the operator norm of $A$ is controlled by the Hilbert-Schmidt norm of $A$
$$\|A\|_{op} \m \|A\|_{HS}$$
\end{lemma}
This result is almost direct in our case ($\|A\|_{op}$ refers to the highest eigenvalue of $A$ and $\|A\|_{HS}$ refers to the square root of the sum of all squared eigenvalues of $A$). For more details, the reader may refer to Chapter 8 in \cite{gohberg2013classes}.
Theorem 1 is sufficient to show $\rho(V_\infty,V_t^p) \tti 0$ thanks to theorem 3 in \cite{zwald2005convergence}. Indeed, we have the following inequality:
$$\rho(V_\infty,V_t^p) \m \frac{\| C_t - C_\infty \|_{op}}{\delta^p}$$
with $\delta^p := \frac{1}{2}( \lambda_\infty^p - \lambda_\infty^{p+1}) = \frac{\lambda_\infty^p}{2}$. The last inequality follows from Assumption 1. The first step is done.

\begin{remark}The same proof works with alternative hypothesis, except that, at the end, $\delta^p = \frac{1}{2}( \lambda_\infty^p - \lambda_\infty^{p+1}) \neq \frac{\lambda_\infty^p}{2}$
\end{remark}
\end{proof}
From the first part, we know that $\|C_t - C_\infty \|_{HS(\mb{H})} \underset{t \rightarrow \infty}{\lra} 0$ and consequently, we know that $\rho(V_\infty,V_t^p) \underset{t \rightarrow \infty}{\lra} 0$. However, quantities in these limit relations are probabilistic quantities and we want to estimate them thanks to a sample $(X_1,...,X_n)$ where the $X_i$'s are i.i.d. as $X$. Hence, we define $\hat{C}_t$ the empirical covariance estimator associated with $(X_1,...,X_n)$ by the following formula
$$\hat{C}_t := \frac{1}{\sum_{l=1}^n \1\{\|X_l\| \s t \}}\sum_{i=1}^n \theta_t (X_i) \otimes \theta_t (X_i) $$
where $\theta(x) := \frac{x}{\|x\|}$.

We also introduce an intermediate quantity to divide the remaining work in two parts. Let $\overline{C}_t$ be the "almost" empirical covariance defined as
$$\overline{C}_t := \frac{1}{\mb{P}(\|X\| \s t )}\sum_{i=1}^n \theta_t (X_i) \otimes \theta_t (X_i) $$

In fact, as mentioned above, the study is divided in two parts since the following inequality holds:
$$\| \hat{C}_{\hat{t}_{n,k}} - C_\infty \|_{HS} \m \| \hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS} + \|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} + \|C_{t_{n,k}}-C_\infty\|_{HS}$$
where $t_{n,k}$ is the quantile of order $1-k/n$ of $\|X\|$ (\emph{i.e.} $\mb{P}(\|X\| \s t_{n,k} ) = k/n$) and $\hat{t}_{n,k}:= \|X_{(k+1)}\|$ is the empirical quantile of order $1-k/n$ of $\|X\|$ (where the $X_{(i)}$'s are such that $\|X_{(1)}\| \s \|X_{(2)}\| \s ...$). One more time, we have to deal with $\hat{t}_{n,k}$  because the true quantile $t_{n,k}$ must be unknown.

The third term of the above inequality is the concern of the first part. Hence, it remains to show
\begin{enumerate}
	\item $\|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} \overset{\mb{P}}{\nti} 0$
	\item $\| \hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS} \overset{\mb{P}}{\nti} 0$
\end{enumerate}
\underline{Remark}: in the following, we will prove more than just the consistency of the estimators by getting concentration bounds for this convergence.
\subsection{$\|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} \overset{\mb{P}}{\nti} 0$}
This part is dedicated to the proof of the following theorem.
\begin{theorem}With probability at least $1- \delta / 2$
$$\|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} \m \frac{1}{\sqrt{k}}+\frac{2}{3k}\log\bigg(\frac{2}{\delta}\bigg)+\bigg(\bigg(\frac{2\log(2/\delta)}{3k}\bigg)^2+\frac{2}{k^2}\log(2/\delta) \bigg)^{1/2}$$
\end{theorem}
\begin{proof}

For convenience, set
$$\fonction{\phi_t}{\mb{H}^n}{\mb{R}}{(x_1,...,x_n)}{\frac{1}{k}\| \sum_{i=1}^n (\theta_t(x_i) \otimes \theta_t(x_i) - \E (\theta_t(X) \otimes \theta_t(X)) \|_{HS}}$$
Notice that $\phi_{t_{n,k}}(X_1,...,X_n)=\|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS}$.
Denote also
$$\E_i\big(\phi_t(x_1,...,x_n)\big) := \E_{Y \sim X} \big(\phi_t(x_1,...,x_{i-1},Y,x_{i+1},...,x_n)\big)$$
$$\sigma_i^2(\phi_t(x_1,...,x_n)) := \frac{1}{2}\E_{(Y,Y') \sim (X,X)} \bigg(\bigg(\phi_t(x_1,...,x_{i-1},Y,x_{i+1},...,x_n)-\phi_t(x_1,...,x_{i-1},Y',x_{i+1},...,x_n)\bigg)^2\bigg)$$
\begin{proposition}
With the above notations, we have
$$\mb{P}(\phi_{t_{n,k}}(X_1,...,X_n) - \E (\phi_{t_{n,k}}(X_1,...,X_n)) \s t ) \m \exp \bigg( \frac{-kt^2}{2(1+\frac{2t}{3})}\bigg)$$
\end{proposition}
\begin{proof}
This proposition only follows from a Bernstein's type inequality (Theorem 3.8 in \cite{mcdiarmid1998concentration}).
Let $(x_1,...,x_n) \in \mb{H}^n$.
\begin{align}
| \phi_{t_{n,k}}(x_1,...,x_n) - \E_i (\phi_{t_{n,k}}(x_1,...,x_n)) | &=
| \E ( \phi_{t_{n,k}}(x_1,...,x_n) - \phi_{t_{n,k}}(x_1,...,x_{i-1},X,x_{i+1},...,x_n) )| \nonumber \\
&\m \frac{1}{k} \E \| \theta_{t_{n,k}}(x_i) \otimes \theta_{t_{n,k}}(x_i)- \theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X) \|_{HS} \nonumber \\
&\m \frac{1}{k}(\1 \{ \|x_i \| \s t_{n,k} \} + \mb{P}( \|X\| \s t_{n,k} )) \m \frac{1+k/n}{k} \m \frac{2}{k} \nonumber
\end{align}
The last bound corresponds to $b$ in \cite{maurer2019bernstein}.

\begin{align}
\sigma_i^2(\phi_t(x_1,...,x_n)) &= \frac{1}{2}\E_{(Y,Y') \sim (X,X)} \bigg(\bigg(\phi_t(x_1,...,x_{i-1},Y,x_{i+1},...,x_n)-\phi_t(x_1,...,x_{i-1},Y',x_{i+1},...,x_n)\bigg)^2\bigg) \nonumber \\
&= \frac{n^2}{k^2} \bigg(\frac{1}{n^2}\E \|\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X)\|_{HS}^2 \nonumber \\
&-\frac{1}{n^2} \E_{(Y,Y') \sim (X,X)} ( \langle \theta_{t_{n,k}}(Y) \otimes \theta_{t_{n,k}}(Y),\theta_{t_{n,k}}(Y') \otimes \theta_{t_{n,k}}(Y')) \bigg) \nonumber \\
&= \frac{1}{k^2}\bigg(\E \|\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X)\|_{HS}^2 - \|\E(\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X))\|_{HS}^2 \bigg) \nonumber \\
&\m \frac{\mb{P}(\|X\| \s t_{n,k})}{k^2}=\frac{1}{nk} \nonumber
\end{align}
Hence, $\sum_{i=1}^n \sigma_i^2(\phi_t(x_1,...,x_n))$ is bounded from above by $1/k$.

Finally, we can apply the Bernstein's type inequality to obtain exactly the wanted inequality.
\end{proof}
\begin{lemma}
$$\E \|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} \m \frac{1}{\sqrt{k}}$$
\end{lemma}
\begin{proof}
\begin{align}
\E \|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} &= \frac{n}{k}\E \bigg\| \frac{1}{n}\sum_{i=1}^n \theta_{t_{n,k}}(X_i)\otimes\theta_{t_{n,k}}(X_i) - \E(\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X) )\bigg\|_{HS} \nonumber \\
&\m \frac{n}{k} \bigg(\E \bigg\| \frac{1}{n}\sum_{i=1}^n \bigg( \theta_{t_{n,k}}(X_i)\otimes\theta_{t_{n,k}}(X_i)  - \E(\theta_{t_{n,k}}(X_i) \otimes \theta_{t_{n,k}}(X_i) )\bigg) \bigg\|_{HS}^2\bigg)^{1/2} \nonumber \\
&\m \frac{n}{k} \bigg( \frac{1}{n} \E \|\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X) - \E(\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X)) \|_{HS}^2 \bigg)^{1/2} \nonumber \\
&= \frac{\sqrt{n}}{k}\bigg( \E \|\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X)\|_{HS}^2 - \| \E ( \theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X))\|_{HS}^2 \bigg)^{1/2} \nonumber \\
&\m \frac{\sqrt{n}}{k}\bigg( \E \|\theta_{t_{n,k}}(X) \otimes \theta_{t_{n,k}}(X)\|_{HS}^2 \bigg)^{1/2} \nonumber \\
&\m \frac{\sqrt{n}}{k}\mb{P}(\|X\| \s t_{n,k})^{1/2} = \frac{1}{\sqrt{k}} \nonumber
\end{align}
For the second inequality, we have used that, for every independent centered random variables $A_i \in \mb{H}, 1 \m i \m n$, one has
$$\E\bigg\|\sum_{i=1}^n A_i \bigg\|_{HS}^2=\sum_{i=1}^n \E\| A_i \|_{HS}^2$$
This assertion follows from $\E \langle A,B \rangle = \langle \E A,\E B \rangle$ if $A \independent B$.

The last inequality follows from $\|\theta(x)\otimes\theta(x)\|_{HS} = 1$.
\end{proof}
Finally, by combining the two above results, we obtain that, with probability at least $1- \delta/2$,
$$\|\overline{C}_{t_{n,k}} - C_{t_{n,k}}\|_{HS} \m \frac{1}{\sqrt{k}}+\frac{2}{3k}\log\bigg(\frac{2}{\delta}\bigg)+\bigg(\bigg(\frac{2\log(2/\delta)}{3k}\bigg)^2+\frac{2}{k^2}\log(2/\delta) \bigg)^{1/2}$$
\end{proof}
\subsection{	$\| \hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS} \overset{\mb{P}}{\nti} 0$}
It is easy to obtain a concentration bound for this term.
\begin{proposition}
$$\mb{P} (\| \hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS} \s t )\m 2 \exp \bigg( \frac{-kt^2}{2(1-k/n+t/3)} \bigg)$$
\end{proposition}
\begin{proof}

First, we have to bound our focused quantity by an easier one.
\begin{align}
\| \hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS} &= 
\frac{1}{k} \| \sum_{i=1}^n \theta(X_i) \otimes \theta(X_i) ( \1\{ \|X_i\| \s t_{n,k} \} -  \1\{ \|X_i\| \s \hat{t}_{n,k} \} ) \|_{HS} \nonumber \\
&\m \frac{1}{k} \sum_{i=1}^n | \1\{ \|X_i\| \s t_{n,k} \} -  \1\{ \|X_i\| \s \hat{t}_{n,k} \} | \nonumber \\
&= \frac{1}{k} \bigg| \sum_{i=1}^n  \1\{ \|X_i\| \s t_{n,k} \} -  k \bigg| \nonumber
\end{align}
The last equality holds since terms in the sum only depend on $\1 \{\hat{t}_{n,k}\s t_{n,k} \}$. Notice that $\sum_{i=1}^n  \1\{ \|X_i\| \s t_{n,k} \}$ follows a binomial distribution with parameter $(n, k/n)$.

Hence, with Bernstein's inequality, we obtain:
\begin{align}
\mb{P} (\| \hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS} \s t ) &\m \mb{P}\bigg(\bigg| \sum_{i=1}^n  \1\{ \|X_i\| \s t_{n,k} \} -  k \bigg| \s kt \bigg) \nonumber \\
&\m 2 \exp \bigg( \frac{-kt^2}{2(1-k/n+t/3)} \bigg) \nonumber
\end{align}
\end{proof}
With the above proposition, we finally obtain, with probability at least $1-\delta/2$
$$\|\hat{C}_{\hat{t}_{n,k}} - \overline{C}_{t_{n,k}} \|_{HS}\m \frac{1}{3k}\log(4/ \delta ) + \bigg( \bigg( \frac{\log (4/\delta)}{3k} \bigg)^2 + \frac{2}{k}(1-k/n)\log(4/ \delta) \bigg)^{1/2}$$
\subsection{Conclusion of the statistical part}
The following theorem is a consequence of proposition 3.1 and proposition 3.2.
\begin{theorem}
With probability at least $1-\delta$
\begin{align}
&\|\hat{C}_{\hat{t}_{n,k}} - C_{t_{n,k}} \|_{HS} \nonumber \\
&\m \frac{1}{\sqrt{k}}+\frac{2}{3k}\log\bigg(\frac{2}{\delta}\bigg)+\bigg(\bigg(\frac{2\log(2/\delta)}{3k}\bigg)^2+\frac{2}{k^2}\log(2/\delta) \bigg)^{1/2} \nonumber \\
&+ \frac{1}{3k}\log(4/ \delta ) + \bigg( \bigg( \frac{\log (4/\delta)}{3k} \bigg)^2 + \frac{2}{k^2}(1-k/n)\log(4/ \delta) \bigg)^{1/2} \nonumber
\end{align}
\end{theorem}
We conclude with theorem 3 of \cite{zwald2005convergence} to obtain
$$\rho(\hat{V}_{\hat{t}_{n,k}},V_{t_{n,k}}) \m \frac{\| \hat{C}_{\hat{t}_{n,k}} - C_{t_{n,k}} \|_{HS}}{\delta^p_{t_{n,k}}}$$
where $\delta^p_{t_{n,k}}:=\frac{1}{2}(\lambda_{t_{n,k}}^p-\lambda_{t_{n,k}}^{p+1})$.
We know by the first part that $||C_t-C_\infty||_{HS} \underset{t \rightarrow \infty}{\lra} 0$. With $| \lambda^p_t - \lambda^p_\infty | \m \|C_t - C_\infty \|_{op}$, we finally deduce that $\delta^p_{t_{n,k}} \nti \delta^p = \frac{\lambda^p_\infty}{2}$ and the proof is over.

Here, concentration bounds are given for estimation of the covariance operator and therefore for estimation of eigenspaces associated with principal components. However, in \cite{blanchard2007statistical} or \cite{drees2021principal}, concentration bounds are given on the reconstruction error. In particular in \cite{blanchard2007statistical}, results are given in general Hilbert spaces setting, which can be applied \emph{mutatis mutandis} here.

==> Simulations.tex <==
%
% We consider regularly varying observations in $L^2([0,1])$ following the same distribution as $X$ such that $X = \sum_{i=1}^{p_1} Y_i f_i+ \sum_{i=p_1 +1}^{p_1 + p_2} W_i f_i$ where $(Y_i)_{1\m i \m p_1}$ are i.i.d. standard Pareto random variable with parameter $\alpha_1$ and $(W_i)_{p_1+1 \m i \m p_1+p_2}$ are i.i.d. following a mean zero normal distribution with same variance $\sigma^2$ as $Y_1$. Hence, $X$ is regularly varying in $\mb{H}$ such that 
%$$L(\frac{X}{\|X\|} | \|X\| > n ) \rightarrow \mathcal{L}(\Theta_\infty)$$
%with $\Theta_\infty \in span\{f_1,f_2\}$ (thresholding crushes normally distributed coordinates).

%We simulate $n=10000$ observations $X_1,...,X_n$ i.i.d. following the same distribution as $X$, with $\alpha_1 = 3$ ($\sigma^2 = 3/4$), $p_1=2$ and $p_2 = 8$. A first principal component analysis on this data does not highlight regularly varying coordinates. Explained variance is evenly distributed over ten principal components. First principal component explains approximately $0.095$ of the total variance and the last principal component explains approximately $0.078$ of the total variance. Figure 1 shows cumulative explained variance.

%\begin{figure}[h]
%    \begin{minipage}[c]{.46\linewidth}
%        \centering
%        \includegraphics[scale = 0.5]{Figure_1.png}
%    \end{minipage}
%    \hfill%
%    \begin{minipage}[c]{.46\linewidth}
%        \centering
 %       \includegraphics[scale = 0.5]{Figure_2.png}
 %   \end{minipage}
%\end{figure}

%Then, we only keep the $k=500$ largest data w.r.t. $\|\cdot\|_2$. Figure 2 shows coordinates according to $f_1,f_2$ of remaining observations. 
%
%Hence, another principal component analysis is released. Explained variance is no longer evenly distributed over principal components. The two first principal components explain more than $0.96$ of the total variance. The first principal component is largely concentrated along $f_1$ and the second principal component along $f_2$. Figure 3 shows cumulative explained variance w.r.t. number of principal component.
%\begin{figure}[h]
%\centering 
%\includegraphics[scale=0.6]{Figure_3.png} 
%\end{figure}

We illustrate that Karhunen-Loève expansion allows us to recover support of a limiting measure derived from a regularly varying random variable. Two models of $L^2([0,1])$-regularly varying random variable are considered where the support of the angular process is concentrated on a $p$-dimensional subspace ($p$ is finite). Methods to generate samples are the same for both processes. Let $(e_i )_{i \s 1}$ be the Fourier orthonormal basis (it can be any basis). We simulate random variables distributed as $X$ where $X$ is given by
\begin{equation}\label{model}
X = \sum_{i \in I_1} Y_i e_i + \sum_{i \in I_2} W_i e_i
\end{equation}
with $I_1,I_2 \subset \bb{N}, I_1 \bigcap I_2 = \emptyset, | I_1 | = p, | I_2 | = d-p, I_1\bigcup I_2 =  \{ 1 ,..., d  \}$ and $(Y_i)_{i \in I_1}$ a regularly varying random vector in $\bb{R}^p$, $(W_i)_{i \in I_2}$ a random vector in $\bb{R}^{p-d}$.
First, we consider a full-independence case with the $Y_i$'s are i.i.d. following Pareto distribution of parameter $\alpha$ and $W_i$'s are i.i.d. following mean-zero normal distribution with variance $\sigma^2$. Second, we consider an extremal-dependence case with $(Y_i)_{i \in I_1}$ following a multivariate logistic model as described in \cite{stephenson2003simulating} and $W_i$'s are i.i.d. following exponential distribution with parameter $\lambda$.

All the studies are done using \emph{scikit-fda} Python package. It allows to represent our data as a basis expansion by stipulate wanted coordinates. Functional principal components analysis is also performed according to a given basis which can be different from the basis used to express our data. In our simulation, we use a Fourier basis to express our data and a BSpline basis to express our principal components.

The same procedure is performed on the two models. First, we generate a sample of $n$ curves and perform a functional principal component analysis on this data after normalization. We examine performances of this procedure by considering reconstruction errors on the first (arbitrary) curves. Then, we keep only the $K$ largest in $L_2([0,1])$-norm curves and we normalize them. A second functional principal component analysis is performed on the remaining sample and we inspect performances according to reconstruction errors while $K$ is varying. In reconstruction error graphs, the first value corresponding to $s = 1$ is always calculated just by removing the mean of the process.

We first discuss results from the Pareto model. We simulate a sample $(X_1,...,X_n)$ of size $n=10.000$ such that
$$X_i = \sum_{j \in I_1} Y_{ij}e_j + \sum_{j \in I_2} W_{ij}e_i$$
with $Y_{ij} \sim Pareto(\alpha)$ and $W_{ij} \sim Norm(0,\sigma^2)$.
We choose different parameters such as $d=11$, $p=3$, $I_1 = \{ 1, 6, 10 \}$ and $\alpha = 3$. We also set $\sigma^2 = 3/4$ in order to have $Var(Y_1) = Var(W_1)$. We deliberately split regularly varying coordinates to enlighten that our procedure does not depend on frequencies associated with coordinates.
\clearpage
\begin{figure}[ht]
\centering
\includegraphics[scale=0.5]{Modele1_Figure1_param(p1,alpha1,p2,alpha2,n,K=3,3,8,np.sqrt(3)2,10000).png}
\centering
\caption{\label{fig:1} Mean (on the $200^{th}$ curves) empirical reconstruction error for PCA, performed on angle of the process without any thresholding, projecting on subspace of dimension $1 \m s \m 11$ versus dimension $s$ for Pareto+Normal model with parameters $\alpha = 3, p = 3$ and $d= 11$.}
\end{figure}
Equal variances of coordinates implies that the process, even normalized, does not concentrate in any particular direction. Hence, principal components must have the same explained variance. In Figure \ref{fig:1}, mean empirical reconstruction error is plotted for principal component procedure on the angle of the sample (\ie normalized sample) but averages are taken only over the $200^{th}$ curves. After removing the mean of our data, it is clear that no principal components stand out from the other due to an almost linear decreasing. Then, only the $k$ observations with the largest $L^2([0,1])$-norm are kept for $k$ varying from $15$ to $200$. Several principal component analysis are done on remaining thresholded samples.

\begin{figure}[ht]
\centering
\includegraphics[scale=0.3]{Modele1_Figure2_param(p1,alpha1,p2,alpha2,n,K=3,3,8,np.sqrt(3)2,10000)_k1-200.png}
\centering
\caption{\label{fig:2} Mean empirical reconstruction errors for PCA, performed on angle of the thresholded process, projecting on subspace of dimension $1 \m s \m 11$ versus $k$ the number of "extremal" curves used for the analysis for Pareto+Normal model with parameters $\alpha = 3, p = 3$ and $d= 11$.}
\end{figure}

In Figure \ref{fig:2}, errors of reconstruction associated to projections on principal eigenspaces of thoses studies are plotted versus $k$. An extremal structure clearly emerges: the three first principal components explain around $0.8$ (depending on the value of $k$) of the process. Since risk plots are close for $p \s 3$, Figure \ref{fig:2} suggests that the support of the angular process is concentrated on a subspace of dimension $p=3$, which is true here by construction. Figure \ref{fig:3} assures "extremal" data and "normal" data have distinct structures by showing an obvious break at $s=3$.
\begin{figure}[ht]
\centering
\includegraphics[scale=0.5]{Modele1_Figure3_param(p1,alpha1,p2,alpha2,n,K=3,3,8,np.sqrt(3)2,10000)_k1-200.png}
\centering
\caption{\label{fig:3} Mean empirical reconstruction errors for PCA, performed on angle of the thresholded process, projecting on subspace of dimension $1 \m s \m 11$ versus $k$ the number of "extremal" curves used for the analysis for Pareto+Normal model with parameters $\alpha = 3, p = 3$ and $d= 11$.}
\end{figure}

The same experiments are realized for the second model. We simulate a sample $(X_1,...,X_n)$ of size $n=10.000$ such that
$$X_i = \sum_{j \in I_{11}} Y_{ij}e_j + \sum_{j \in I_{12}} Y_{ij}e_j + \sum_{j \in I_2} W_{ij}e_i$$
with $(Y_{ij})_{j \in I_11}$ and $(Y_{ij})_{j \in I_11}$ independent distributed with a Gumbel copula \ie with joint distribution function $C_\eta (x) = \exp \Big(-\big( \sum_{j \in I_1} (-\log x_j)^\eta \big)^{1/\eta} \Big)$, where $\eta \in [1,+\infty[$ characterizes the dependence between coordinates, and Fréchet marginals with parameter $\alpha$ and $W_{ij} \sim Norm(0,\sigma^2)$.

We choose different parameters such as $d = 15$, $p=4$, $I_{11} = \{2,7 \}$, $I_{12} = \{ 8, 12\}$ and $\alpha = 2.5$. We also set $\sigma^2 = 1.5$ in such a way that each coordinate has the same variance (which implies no preferential direction for variance without any thresholding). We set the dependence parameter $\nu = 0.1$ which lead to an important dependence between coordinates for extremal data. Hence, extremes are mostly concentrated on the diagonal between $e_2$ and $e_7$ and on the diagonal between $e_8$ and $e_{12}$ which form a subspace of dimension $2$. As for the first simulation, Figure \ref{fig:4} shows no preferential direction even if a the first little break at $s=1$ attests that the mean of the data have more weight in reconstruction error than the principal components.
\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{Modele2_Figure1_param(p1,alpha1,p2,alpha2,n,K,dep_index=4,2.5,11,np.sqrt(1.5),10000,200,0.1)_doublelogmod.png} 
\centering
\caption{\label{fig:4} Mean (on the $200$ first curves) empirical reconstruction error for PCA, performed on angle of the process without any thresholding, projecting on subspace of dimension $1 \m s \m 15$ versus dimension $s$ for DoubleLogMod+Norm model with parameters $\alpha = 2.5, p = 4$ and $d= 15$.}
\end{figure}

Hence, the same plots than for the first simulation is done. Figure \ref{fig:5} corresponds to mean empirical reconstruction errors after thresholding and normalization of the data in according to $k$, the number of curves kept for the analyses. The result is evident and recommend that the dimension of regularly varying part of the data is two. Notice that the dependence between extreme data is too important to detect the two other directions where extremes appear. It is also interesting to notice that in Figure \ref{fig:2} and \ref{fig:5} the last principal components are of growing importance when $k$ grows up; the only reason is when $k$ increases the data tend to become again data without thresholding which implies that the principal components almost contain the same amount of information.
\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{Modele2_Figure2_param(p1,alpha1,p2,alpha2,n,K,dep_index=4,2.5,11,np.sqrt(1.5),10000,200,0.1)_doublelogmod.png} 
\centering
\caption{\label{fig:5} Mean empirical reconstruction errors for PCA, performed on angle of the thresholded process, projecting on subspace of dimension $1 \m s \m 15$ versus $k$ the number of "extremal" curves used for the analysis for DoubleLogMod+Norm model with parameters $\alpha = 2.5, p = 4$ and $d= 15$.}
\end{figure}

Figure \ref{fig:6} corresponds to the mean empirical reconstruction error for $k = 100$ and again, the break at $s = 2$ is obvious.
\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{Modele2_Figure3_param(p1,alpha1,p2,alpha2,n,K,dep_index=4,2.5,11,np.sqrt(1.5),10000,200,0.1)_doublelogmod.png} 
\centering
\caption{\label{fig:6} Mean empirical reconstruction error for PCA performed on angle of the thresholded process keeping $k=100$ curves, projecting on subspace of dimension $1 \m s \m 15$ versus dimension $s$ for DoubleLogMod+Expon model with parameters $\alpha = 2.5, p = 4$ and $d= 15$.}
\end{figure}

To sum up, when dealing with regularly varying data, if extreme data are considered, principal components on the whole data set may be irrelevant. However, principal components analyses on thresholded and normalized data catches important amount of information and seems to well-determines the dimension of the subspace onto regularly varying coordinates belong.

==> abstractEVA.tex <==
We develop a general probabilistic and statistical framework 
for low dimensional projections of extremes of regularly  varying  stochastic processes $X_t, t\in [0,1]$    with square integrable trajectories,  \textit{i.e.} $L^2([0,1])$. Our goal is to propose a dimension reduction framework allowing to handle extreme data  of functional nature, which are increasingly available in the  IoT and Big Data era, with various applications such as the predictive maintenance of sophisticated systems (\textit{e.g.} energy networks, aircraft fleet) through anomaly detection. We propose a notion of  Karuhnen-Loeve (KL) expansion accounting  for the principal `directions' of functional extremes, understood in the sense  of peaks-over-threshold for the $L^2$ norm. 
Following in the footstep of PCA for multivariate extremes, but differently from existing work regarding KL of regularly varying processes, our focus   of the `angular' component of extreme functions.  This reduction to a bounded sample space automatically enforces   moments assumptions which  are mathematically convenient when handling covariance operators.   We investigate the statistical properties of  the empirical KL expansion of this angular process, by upper-bounding the Hilbert-Schmidt norm of the error of the empirical covariance operator for finite sample sizes. Numerical experiments illustrate this work. 


%We first extend the notion of regular variation to stochastic processes $X$ indexed by $t\in[0,1]$ with square integrable trajectories, \textit{i.e.} s.t. $\int_0^1X^2(t)dt<+\infty$ with probability one.

==> todo.tex <==
\textbf{A lire pour les applis (les plus cités/récents):}voir \ref{wang2008karhunen} pour une review très complète sur KLE et sur qq applis
\begin{itemize}
	\item PCA/KLE clustering ($K$-means clustering equivalent to PCA \cite{ding2004k});
	\item PCA/KLE detection/prediction;
	\item simulation de nouvelles données grâce à ACP (intérêt? image?): application en geostats (\ref{zheng2017simulation}) simuler le random field limite mais il faut connaissance de la fonction de cov et de les loi marginale du processus initial;
	\item comparer avec les travaux déjà faits avec KLE (ou PCA sur dataset discrétisé);
	\item comparer avec travaux extrêmes (spatials?).
	\item regression fonctionnelle dans les extremes;
	\item etendre les resultats aux espaces de sobolev: plus général, pas très couteux
\end{itemize}

\textbf{Pour trouver un dataset:}
\begin{itemize}
	\item A multivariate extreme value theory approach to anomaly clustering and visualization;
	\item dataset Kokozska/Xiong;
	\item jeu de données environnemental (température/précipitation);
	\item demander Guillaume/Dimitri;
	\item dataset avec anomalies simulées rajoutées (moins d'intérêt).
\end{itemize}

\textbf{Manquant dans l'article:}
\begin{itemize}
	\item exemple génératif: solution d'une EDP, modèle ARMA/GARCH (pas selon une base) (regarder dans \cite{FDA});

	\item obtenir des garanties pour des données discrtisées?
\end{itemize}
